Extended Plefka Expansion for Stochastic Dynamics

We propose an extension of the Plefka expansion, which is well known for the dynamics of discrete spins, to stochastic differential equations with continuous degrees of freedom and exhibiting generic nonlinearities. The scenario is sufficiently general to allow application to e.g. biochemical networks involved in metabolism and regulation. The main feature of our approach is to constrain in the Plefka expansion not just first moments akin to magnetizations, but also second moments, specifically two-time correlations and responses for each degree of freedom. The end result is an effective equation of motion for each single degree of freedom, where couplings to other variables appear as a self-coupling to the past (i.e. memory term) and a coloured noise. This constitutes a new mean field approximation that should become exact in the thermodynamic limit of a large network, for suitably long-ranged couplings. For the analytically tractable case of linear dynamics we establish this exactness explicitly by appeal to spectral methods of Random Matrix Theory, for Gaussian couplings with arbitrary degree of symmetry.

==> pstricks.tex <==
%% pstricks.tex
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%% COPYRIGHT 2000-2003 by Denis Girou.
%% Copyright 2004-2015 Herbert Voss
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2003/12/01 or later.
%
% This work has the LPPL maintenance status "maintained".
% 
% This Current Maintainer of this work is Herbert Voss
%
\csname PSTricksLoaded\endcsname
\let\PSTricksLoaded\endinput  
%
%% !! loading additional TeX packages see line 112 !!
%% !! loading config file pstricks.con    line 476 !!
%% !! loading pro files                   line 489 !!
%% !! fileversion and date see            line 119 !!
%
\edef\PstAtCode{\the\catcode`\@}
\catcode`\@=11\relax
%
\expandafter\ifx\csname @latexerr\endcsname\relax%	do we have LaTeX?
  \def\typeout#1{\immediate\write\@unused{#1}}%
  \gdef\ch@ck#1#2#3{\ifnum\count1#1<#2 \else\errmessage{No room for a new #3}\fi}
  \countdef\allocationnumber=21
  \chardef\sixt@@n=16
  \def\alloc@#1#2#3#4#5{\global\advance\count1#1\@ne
    \ch@ck#1#4#2% make sure there's still room
    \allocationnumber\count1#1%
    \global#3#5\allocationnumber
    \wlog{\string#5=\string#2\the\allocationnumber}}
  \alloc@7\write\chardef\sixt@@n\@unused
  \typeout{we are running tex and have to define some LaTeX commands ...}%
  \long\def\@ifundefined#1#2#3{\expandafter\ifx\csname #1\endcsname\relax#2\else#3\fi}
  \def\@namedef#1{\expandafter\def\csname #1\endcsname}
  \def\@nameuse#1{\csname #1\endcsname}
  \def\@eha{%
    Your command was ignored.^^J
    Type \space I <command> <return> \space to replace
    it with another command,^^J
    or \space <return> \space to continue without it.}
  \def\@spaces{\space\space\space\space}
  \def\@empty{}
  \def\@gobble#1{}
  \def\@nnil{\@nil}
%
  \def\@ifnextchar#1#2#3{%
    \let\@tempe#1\def\@tempa{#2}\def\@tempb{#3}\futurelet\@tempc\@ifnch}
%
  \def\@ifnch{%
    \ifx\@tempc\@sptoken \let\@tempd\@xifnch
    \else\ifx\@tempc\@tempe \let\@tempd\@tempa \else \let\@tempd\@tempb \fi
    \fi
    \@tempd%
  }
  \begingroup
  \def\:{\global\let\@sptoken= } \:
  \def\:{\@xifnch} \expandafter\gdef\: {\futurelet\@tempc\@ifnch}
  \endgroup
  \def\endtabular{\crcr\egroup\egroup $\egroup}
  \def\@width{width}% needed by pst-node
  \def\@tfor#1:={\@tf@r#1 }
  \long\def\@tf@r#1#2\do#3{\def\@fortmp{#2}\ifx\@fortmp\space\else
     \@tforloop#2\@nil\@nil\@@#1{#3}\fi}%
  \long\def\@tforloop#1#2\@@#3#4{\def#3{#1}\ifx #3\@nnil
       \expandafter\@fornoop \else
      #4\relax\expandafter\@tforloop\fi#2\@@#3{#4}}
  \long\def\@break@tfor#1\@@#2#3{\csname fi\endcsname\csname fi\endcsname}
\fi%
\catcode`\@=\PstAtCode\relax
%
% now we have all commands defined, for TeX and LaTeX
%
\ifx\PSTXKeyLoaded\endinput\else \input pst-xkey.tex \fi
\catcode`\@=11\relax
\def\XKV@ch@ckch@ice#1#2#3{%  bugfix for xkeyval
  \def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@nnil\let\XKV@tempa\@empty\else
    \def\XKV@tempa{\def#1{#2}}%
  \fi
%  \in@{,#2,}{,#3,}%
\begingroup\edef\x{\endgroup\noexpand\in@{,#2,}}\x{,#3,}%
%\expandafter\in@\expandafter{\expandafter,#2,}{,#3,}% --- hv 2012-04-27
  \ifin@
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@firstoftwo
    \else
      \XKV@addtomacro@n\XKV@tempa\@firstofone
    \fi
  \else
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@secondoftwo
    \else
      \XKV@toks{#2}%
      \XKV@err{value `\the\XKV@toks' is not allowed}%
      \XKV@addtomacro@n\XKV@tempa\@gobble
    \fi
  \fi
  \XKV@tempa
}

\def\ProvidesPackageRCS{\@ifnextchar[\ProvidesPackageRCS@i{\ProvidesPackageRCS@i[] }}  %$
\def\ProvidesPackageRCS@i[#1] $#2${} %$
\catcode`\@=\PstAtCode\relax
\ifx\PSTFPloaded\endinput\else   \input pst-fp.tex\fi

\input pgfutil-common.tex
\input pgfkeys.code.tex
\input pgffor.code.tex
\let\pgfforeach\foreach
%
\def\fileversion{2.63}
\def\filedate{2015/09/11}
\catcode`\@=11\relax
\pst@addfams{pstricks}
%
% stolen from latex.ltx to make it TeX compatible
\newcount\psLoopIndex
\def\@fornoop#1\@@#2#3{}
\long\def\@for#1:=#2\do#3{%
  \pst@cntm=0
  \expandafter\def\expandafter\@fortmp\expandafter{#2}%
  \ifx\@fortmp\@empty \else
    \expandafter\@forloop#2,\@nil,\@nil\@@#1{#3}\fi}
%
\long\def\@forloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx#4\@nnil \else
       #5\def#4{#2}\ifx#4\@nnil \else\global\advance\psLoopIndex by \@ne\relax
       #5\@iforloop #3\@@#4{#5}\fi\fi}

\long\def\@iforloop#1,#2\@@#3#4{\global\advance\psLoopIndex by \@ne\relax%
   \def#3{#1}\ifx #3\@nnil
     \expandafter\@fornoop \else
     #4\relax\expandafter\@iforloop\fi#2\@@#3{#4}}
%
\long\def\psforeach#1#2#3{%
  \global\psLoopIndex=0\relax
  \if$\ifnum9<1#2$\else\fi\psforeach@ii{#1}{#2}{#3}%
  \else                      \expandafter\psforeach@i#2,..,,..,\@nil{#1}{#3}\fi}
\long\def\psforeach@i#1,#2,..,#3,..,#4\@nil#5#6{% 
  \ifx\relax#3\relax\psforeach@ii{#5}{#1,#2}{#6}%
  \else\psforeach@iii{#5}{#1}{#2}{#3}{#6}\fi}
\long\def\psforeach@ii#1#2#3{%
  \begingroup
  \edef\reserved@a{#2}%
  \@for#1:=\reserved@a\do{#3}%
  \endgroup}
\long\def\psforeach@iii#1#2#3#4#5{%
  \pstFPsub\pst@tempA{#3}{#2}%
  \pst@dimm=\pst@tempA pt%
  \pstFPstripZeros{\pst@tempA}\pst@tempB%
  \def\pst@tempA{#2}%
  \def\pst@tempa{#2}%
  \pst@dimn=#4pt%
  \loop
    \pst@dimm=\pst@tempA pt
    \ifdim\pst@dimm<\pst@dimn
      \pstFPadd\pst@tempA{\pst@tempA}{\pst@tempB}%
      \pstFPstripZeros{\pst@tempA}\pst@tempA%
      \edef\pst@tempa{\pst@tempa,\pst@tempA}%
  \repeat%
  \psforeach@ii{#1}{\pst@tempa}{#5}}
%
\long\def\psForeach#1#2#3{%  without grouping the contents
  \global\psLoopIndex=0\relax%
  \if$\ifnum9<1#2$\else\fi\psforeach@ii{#1}{#2}{#3}%
  \else                   \expandafter\psForeach@i#2,..,,..,\@nil{#1}{#3}\fi}
\long\def\psForeach@i#1,#2,..,#3,..,#4\@nil#5#6{% 
  \ifx\relax#3\relax\psForeach@ii{#5}{#1,#2}{#6}%
  \else\psForeach@iii{#5}{#1}{#2}{#3}{#6}\fi%
}
\long\def\psForeach@ii#1#2#3{%
  \edef\reserved@a{#2}%
  \@for#1:=\reserved@a\do{#3}}
\long\def\psForeach@iii#1#2#3#4#5{%
  \pstFPsub\pst@tempA{#3}{#2}%
  \pst@dimm=\pst@tempA pt%
  \pstFPstripZeros{\pst@tempA}\pst@tempB%
  \def\pst@tempA{#2}%
  \def\pst@tempa{#2}%
  \pst@dimn=#4pt%
  \loop%
    \pst@dimm=\pst@tempA pt%
    \ifdim\pst@dimm<\pst@dimn%
      \pstFPadd\pst@tempA{\pst@tempA}{\pst@tempB}%
      \pstFPstripZeros{\pst@tempA}\pst@tempA
      \edef\pst@tempa{\pst@tempa,\pst@tempA}%
  \repeat%
  \psForeach@ii{#1}{\pst@tempa}{#5}
}
  
\def\psrecur@i#1{\csname ps@rn#1\psrecur@i} 
\long\def\ps@rnm#1{\endcsname{#1}#1\global\advance\psLoopIndex by \@ne}
\long\def\ps@rn#1{}
\def\psLoop#1{\global\psLoopIndex=0\relax%
  \csname ps@rn\expandafter\psrecur@i
  \romannumeral\number\number#1 000\endcsname\endcsname}

%
% hv 2007-10-16 to fix the bug in pst-node with \\[name=...]
% hv fix bug with empty fnodes in psmatrix
\def\ps@ifnextchar#1#2#3{%
  \let\reserved@d= #1%
  \def\reserved@a{#2}\def\reserved@b{#3}%
  \futurelet\@let@token\ps@ifnch}
\def\ps@ifnch{%
  \ifx\@let@token\reserved@d \let\reserved@b\reserved@a \fi
  \reserved@b
}
\def\pshskip#1{\vrule \@width\z@\nobreak \hskip #1\hskip \z@skip}
% end bugfix
\typeout{`PSTricks' v\fileversion\space\space <\filedate> (tvz)}
\def\@pstrickserr#1#2{%
  \begingroup
  \newlinechar`\^^J
  \edef\pst@tempc{#2}%
  \expandafter\errhelp\expandafter{\pst@tempc}%
  \typeout{%
    PSTricks error. \space See User's Guide for further information.^^J
    \@spaces\@spaces\@spaces\@spaces
    Type \space H <return> \space for immediate help.}%
  \errmessage{#1}%
  \endgroup}
\def\@ehpa{%
  Your command was ignored. Default value substituted.^^J
  Type \space <return> \space to procede.}
\def\@ehpb{%
  Your command was ignored. Will recover best I can.^^J
  Type \space <return> \space to procede.}
\def\@ehpc{%
  You better fix this before proceding.^^J
  See the PSTricks User's Guide or ask your system administrator for help.^^J
  Type \space X <return> \space to quit.}
\def\@ehpd{%
  Not allowed optional argument.^^J
  Will proceed with the default setting.^^J
  Type \space X <return> \space to quit.}
\def\pst@misplaced#1{\@pstrickserr{Misplaced \string#1 command}\@ehpb}
\newdimen\pst@dima
\newdimen\pst@dimb
\newdimen\pst@dimc
\newdimen\pst@dimd
\newdimen\pst@dimg
\newdimen\pst@dimh
\newdimen\pst@dimm
\newdimen\pst@dimn
\newdimen\pst@dimo
\newdimen\pst@dimp
\chardef\f@ur=4
%
\newbox\pst@hbox
\newbox\pst@ibox
\newbox\pst@boxg
\newcount\pst@cnta
\newcount\pst@cntb
\newcount\pst@cntc
\newcount\pst@cntd
\newcount\pst@cntg
\newcount\pst@cnth
\newcount\pst@cntm
\newcount\pst@cntn
\newcount\pst@cnto
\newcount\pst@cntp
\newcount\@zero\@zero=0\relax
%
\newif\ifPst@SpecialLength
\Pst@SpecialLengthfalse
%
\newif\if@pst
\newtoks\pst@toks
\newif\if@star
\def\pst@ifstar#1{%
  \@ifnextchar*{\@startrue\def\ps@next*{#1}\ps@next}{\@starfalse#1}}
%
\def\pst@expandafter#1#2{%
  \def\ps@next{#1}%
  \edef\@tempa{#2}%
  \ifx\@tempa\@empty
    \@pstrickserr{Unexpected empty argument!}\@ehpb
    \def\@tempa{\@empty}%
  \fi
  \expandafter\ps@next\@tempa}
%
\def\pst@dimtonum#1#2{\edef#2{\pst@@dimtonum#1}}
\def\pst@@dimtonum#1{\expandafter\pst@@@dimtonum\the#1}
{\catcode`\p=12 \catcode`\t=12 \global\@namedef{pst@@@dimtonum}#1pt{#1}}
%
\def\pst@getdimdim#1 #2 #3\@nil{%
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty
    \pssetlength\pst@dimn{#1}%
    \pst@dimm=\z@%
  \else%
    \pssetlength\pst@dimm{#1}%
    \pssetlength\pst@dimn{#2}%
  \fi%
}
\def\pst@getxdimdim#1 #2 #3\@nil{%
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty
    \pssetxlength\pst@dimn{#1}%
    \pst@dimm=\z@
  \else%
    \pssetxlength\pst@dimm{#1}%
    \pssetxlength\pst@dimn{#2}%
  \fi%
}
\def\pst@getydimdim#1 #2 #3\@nil{%
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty
    \pssetylength\pst@dimn{#1}%
    \pst@dimm=\z@%
  \else
    \pssetylength\pst@dimm{#1}%
    \pssetylength\pst@dimn{#2}%
  \fi}
%
% A modulo macro for integer values
% \pst@mod{34}{6}\value ==> \value is 4
%
\def\pst@mod#1#2#3{%
  \begingroup%
  \pst@cntm=#1\pst@cntn=#2\relax%
  \pst@cnto=\pst@cntm%
  \divide\pst@cntm by \pst@cntn%
  \multiply\pst@cntn by \pst@cntm%
  \advance\pst@cnto by -\pst@cntn%
  \edef\value{\endgroup\def\noexpand#3{\number\pst@cnto}}\value%
}
\def\pst@max#1#2#3{%
  \begingroup%
  \pst@cntm=#1\pst@cntn=#2\relax%
  \ifnum\pst@cntm<\pst@cntn\pst@cntm=\pst@cntn\fi
  \global#3=\the\pst@cntm%
  \endgroup%
}
\def\pst@maxdim#1#2#3{%
  \begingroup%
  \pst@dimm=#1\pst@dimn=#2\relax%
  \ifdim\pst@dimm<\pst@dimn\pst@dimm=\pst@dimn\fi
  \global#3=\the\pst@dimm%
  \endgroup%
}
\def\pst@mindim#1#2#3{%
  \begingroup%
  \pst@dimm=#1\pst@dimn=#2\relax%
  \ifdim\pst@dimm>\pst@dimn\pst@dimm=\pst@dimn\fi
  \global#3=\the\pst@dimm%
  \endgroup%
}
\def\pst@abs#1#2{%
  \begingroup%
  \pst@cntm=#1\relax%
  \ifnum\pst@cntm<\z@\pst@cntm=-\pst@cntm\fi%
  \global#2=\the\pst@cntm
  \endgroup%
}
\def\pst@absdim#1#2{%
  \begingroup%
  \pst@dimm=#1\relax%
  \ifdim\pst@dimm<\z@\pst@dimm=-\pst@dimm\fi%
  \global#2=\the\pst@dimm%
  \endgroup%
}
%
\def\pst@pyth#1#2#3{% from pst-3d
  \begingroup%
    \pst@dima=#1\relax%
    \ifnum\pst@dima<\z@\pst@dima=-\pst@dima\fi% dima=abs(x)
    \pst@dimb=#2\relax%
    \ifnum\pst@dimb<\z@\pst@dimb=-\pst@dimb\fi% dimb=abs(y)
    \advance\pst@dimb\pst@dima         % dimb=s=abs(x)+abs(y)
    \ifnum\pst@dimb=\z@
      \global\pst@dimg=\z@             % dimg=z=sqrt(x^2+y^2)
    \else
      \multiply\pst@dima 8\relax              % dima= 8abs(x)
      \pst@@divide\pst@dima\pst@dimb     % dimg =8t=8abs(x)/s
      \advance\pst@dimg -4pt            % dimg = 4tau = (8t-4)
      \multiply\pst@dimg 2
      \pst@dimtonum\pst@dimg\pst@tempa
      \pst@dima=\pst@tempa\pst@dimg           % dima=(8tau)^2
      \advance\pst@dima 64pt         % dima=u=[64+(8tau)^2]/2
      \divide\pst@dima 2\relax                      % =(8f)^2
      \pst@dimd=7pt                % initial guess at sqrt(u)
      \pst@@pyth\pst@@pyth\pst@@pyth            % dimd=sqrt(u)
      \pst@dimtonum\pst@dimd\pst@tempa
      \pst@dimg=\pst@tempa\pst@dimb
      \global\divide\pst@dimg 8             % dimg=z=(8f)*s/8
    \fi
  \endgroup
  #3=\pst@dimg}
%
\def\pst@@pyth{%                      dimd = g <-- (g + u/g)/2
  \pst@@divide\pst@dima\pst@dimd
  \advance\pst@dimd\pst@dimg
  \divide\pst@dimd 2\relax}
%
% ----- the old pst@pyth begin -----  did not use dimens
\def\pst@Pyth#1#2#3{\ifdim#1>#2\pst@@Pyth#1#2#3\else\pst@@Pyth#2#1#3\fi}
\def\pst@@Pyth#1#2#3{%
  \ifdim4#1>9#2\relax
    #3=#1\advance#3 .2122#2%
  \else
    #3=.8384#1\advance#3 .5758#2%
  \fi%
}
% ----- the old pst@pyth end -----
%
%------ new version \pst@divide ̣-------- by Michael Sharpe
\def\pst@divide#1#2#3{%
  \pst@@divide{#1}{#2}%
  \advance\pst@dimg \pst@cnta pt%
  \pst@dimtonum\pst@dimg{#3}%
}
\def\pst@@divide#1#2{%
  \pst@dimg=#1\relax%
  \pst@dimh=#2\relax%
  \pst@cnth=\pst@dimh%
  \pst@cntg=\pst@dimg%
  \pst@cnta=\pst@cntg%
  \divide\pst@cnta\pst@cnth%
  \advance\pst@dimg -\pst@cnta\pst@dimh%
  \pst@cntm=67108863\relax %2^26 -1
  \pst@@@divide\pst@@@divide\pst@@@divide\pst@@@divide%
  \divide\pst@dimg\pst@cnth%
}%
\def\pst@@@divide{%
  \ifnum%
    \ifnum\pst@dimg<\z@-\fi\pst@dimg<\pst@cntm%
      \multiply\pst@dimg\sixt@@n%
  \else%
    \divide\pst@cnth\sixt@@n%
  \fi%
}%
%
%-------------- the old version ----------
\iffalse
\def\pst@divide#1#2#3{%
  \pst@@divide{#1}{#2}%
  \pst@dimtonum\pst@dimg{#3}%
}
\def\pst@@divide#1#2{%
  \pst@dimg=#1\relax
  \pst@dimh=#2\relax
  \pst@cntg=\pst@dimh
  \pst@cnth=67108863
  \pst@@@divide\pst@@@divide\pst@@@divide\pst@@@divide
  \divide\pst@dimg\pst@cntg%
}
\def\pst@@@divide{%
  \ifnum
    \ifnum\pst@dimg<\z@-\fi\pst@dimg<\pst@cnth
      \multiply\pst@dimg\sixt@@n
    \else
      \divide\pst@cntg\sixt@@n
    \fi%
}
\fi
%-------------- end old vesrion ---------------
%
\def\pst@configerr#1{\@pstrickserr{\string#1 not defined in pstricks.con}\@ehpc}
%
\def\pstVerb#1{\pst@configerr\pstVerb}
\def\pstverb#1{\pst@configerr\pstverb}
\def\pstverbscale{\pst@configerr\pstverbscale}
\def\pstrotate{\pst@configerr\pstrotate}
\def\pstheader#1{\pst@configerr\pstheader}
\def\pstdriver{\pst@configerr\pstdriver}
\@ifundefined{pstcustomize}%
  {\def\pstcustomize{\endinput\let\pstcustomize\relax}}{}
%
\input pstricks.con		% local config file
%
\newif\ifPSTricks
\PSTrickstrue
\def\PSTricksOff{%
  \def\pstheader##1{}%
  \def\pstverb##1{}%
  \def\pstVerb##1{}%
  \PSTricksfalse%
}
\@ifundefined{pst@def}{\def\pst@def#1<#2>{\@namedef{tx@#1}{#2 }}}{}
\@ifundefined{pst@ATH}{\def\pst@ATH<#1>{}}{}
%
\pstheader{pstricks.pro}
\pstheader{pst-algparser.pro}
\pstheader{pst-tools.pro}
%
\def\pst@dict{tx@Dict begin }
\def\pst@theheaders{pstricks.pro, pst-algparser.pro}
\def\pst@Verb#1{\pstVerb{\pst@dict #1 end}}
\def\tx@Atan{Atan }
\def\tx@Div{Div }
\def\tx@NET{NET }
\def\tx@Pyth{Pyth }
\def\tx@PtoC{PtoC }
\def\tx@PathLength@{PathLength@ }
\def\tx@PathLength{PathLength }
\pst@dimg=\pstunit\relax
\ifdim\pst@dimg=1bp
\def\pst@stp{.996264 dup scale}
\else
\edef\pst@stp{1 \pst@@dimtonum\pst@dimg\space div dup scale}
\fi
\def\tx@STP{STP }
\def\tx@STV{STV }
%
%--------------------------------------- PS stuff ---------------------------------
% on stack x y 
\pst@def{UserCoor}< \pst@number\psyunit div exch \pst@number\psxunit div exch >
\pst@def{ScreenCoor}< \pst@number\psyunit mul exch \pst@number\psxunit mul exch >
%--------------------------------------- PS stuff end -----------------------------
%
\def\pst@number#1{\pst@@dimtonum#1\space}
%
%-----------------------% hv 20100413
\def\pst@strip@dot#1{\expandafter\pst@strip@dot@i#1..\@nil}
\def\pst@strip@dot@i#1.#2.#3\@nil{%
  \ifnum1#2>10\relax #1.#2\else#1\fi}
%-----------------------% hv 20100413
\def\pst@checknum#1#2{%
  \edef\ps@next{#1}%
  \ifx\ps@next\@empty\let\pst@num\z@%
  \else\expandafter\pst@@checknum\ps@next..\@nil%
  \fi%
  \ifcase\pst@num%  0
    \@pstrickserr{Bad number: `#1'. 0 substituted.}\@ehpa%
    \def#2{0 }%
  \or%              1
    \edef#2{\ifnum\pst@num=\tw@-\fi\the\pst@cntg.%
      \expandafter\@gobble\the\pst@cnth\space}%
  \or%              2
    \edef#2{\ifnum\pst@num=\tw@-\fi\the\pst@cntg.%
      \expandafter\@gobble\the\pst@cnth\space}%
  \or%              3
    \edef#2{\pst@tempA\space}%
  \fi}
\def\pst@@checknum{%
  \@ifnextchar-%
  {\let\pst@num\tw@\expandafter\pst@@@checknum\@gobble}%
  {\@ifnextchar !%
    {\def\pst@num{3}\pst@@@@@checknum}
    {\let\pst@num\@ne\pst@@@checknum}}%
}
\def\pst@@@checknum#1.#2.#3\@nil{%
\afterassignment\pst@@@@checknum\pst@cntg=0#1\relax\@nil%
\afterassignment\pst@@@@checknum\pst@cnth=1#2\relax\@nil}
\def\pst@@@@checknum#1\relax\@nil{\ifx\@nil#1\@nil\else\let\pst@num\z@\fi}
%
\def\pst@@@@@checknum#1#2.#3\@nil{\def\pst@tempA{#2}}% PostScript Notation with !<code>
%
\def\pst@getnumii#1 #2 #3\@nil{%
  \pst@checknum{#1}\pst@tempg%
  \ifx\relax#2\relax\let\pst@temph\pst@tempg\else\pst@checknum{#2}\pst@temph\fi}
\def\pst@getnumiii#1 #2 #3 #4\@nil{%
\pst@checknum{#1}\pst@tempg%
\pst@checknum{#2}\pst@temph%
\pst@checknum{#3}\pst@tempi}
\def\pst@getnumiv#1 #2 #3 #4 #5\@nil{%
\pst@checknum{#1}\pst@tempg%
\pst@checknum{#2}\pst@temph%
\pst@checknum{#3}\pst@tempi%
\pst@checknum{#4}\pst@tempj}
%
\def\pst@getdimnum#1 #2 #3\@nil{%
  \pssetlength\pst@dimg{#1}%
  \pst@checknum{#2}\pst@tempg%
}
\def\pst@getscale#1#2{%	read and check a scale input x [y]
  \edef\pst@tempg{#1}%
  \ifx\pst@tempg\@none
    \def#2{}%
  \else
    \pst@expandafter\pst@getnumii{#1 #1} {} {} {}\@nil
    \ifdim\pst@tempg\p@=\z@
      \@pstrickserr{Bad scaling argument `#1'}\@ehpa
      \def#2{}%
    \else
      \ifdim\pst@temph\p@=\z@
        \@pstrickserr{Bad scaling argument `#1'}\@ehpa
        \def#2{}%
      \else
        \edef#2{\pst@tempg\space \pst@temph\space scale }%
      \fi
    \fi
  \fi%
}
\def\pst@getint#1#2{%	read and check an integer
  \pst@cntg=#1\relax
  \edef#2{\the\pst@cntg\space}%
}
\begingroup
\catcode`\{=12
\catcode`\}=12
\catcode`\[=1
\catcode`\]=2
\gdef\pslbrace[{ ]
\gdef\psrbrace[} ]
\endgroup

\pstVerb{
  /pssetRGBcolor  /setrgbcolor  load def
  /pssetCMYKcolor /setcmykcolor load def
  /pssetGraycolor /setgray      load def
}
\def\@newcolor#1#2{%
  \expandafter\edef\csname #1\endcsname{\noexpand\pst@color{#2}}%
  %\expandafter\edef\csname color@#1\endcsname{#2}%
  \expandafter\edef\csname\string\color@#1\endcsname{#2}%    hv 1.14 2005-12-17
  \ignorespaces}
\def\pst@color#1{%
  \def\pst@currentcolor{#1}\pstVerb{#1}\aftergroup\pst@endcolor}%
\def\pst@endcolor{\pstVerb{\pst@currentcolor}}
\def\pst@currentcolor{0 setgray}
\def\altcolormode{%
\def\pst@color##1{%
  \pstVerb{gsave ##1}\aftergroup\pst@endcolor}%
\def\pst@endcolor{\pstVerb{\pst@grestore}}}
\def\pssetMonochrome{%
  \pstVerb{
    /setrgbcolor { add add 0 gt {0}{1} ifelse setgray } def 
    /setcmykcolor{ 4 dict begin
      /k ED /y ED /m ED /c ED 
      1 1 k sub c mul k add sub 0.29 mul 
      1 1 k sub m mul k add sub 0.587 mul add 
      1 1 k sub y mul k add sub 0.114 mul add
      end 0 gt {0}{1} ifelse setgray } def }}
\def\pssetGrayscale{%
  \pstVerb{
    /setrgbcolor { 0.07 mul exch 0.71 mul add exch 0.21 mul add setgray } def 
    /setcmykcolor{ 4 dict begin
      /k ED /y ED /m ED /c ED 
      1 1 k sub c mul k add sub 0.29 mul 
      1 1 k sub m mul k add sub 0.587 mul add 
      1 1 k sub y mul k add sub 0.114 mul add
      end setgray } def }}
\def\psresetColor{\pstVerb{
    /setrgbcolor  tx@Dict begin /pssetRGBcolor  load end def 
    /setcmykcolor tx@Dict begin /pssetCMYKcolor load end def }}

\def\pst@grestore{
  currentpoint
  matrix currentmatrix
  currentfont
  grestore
  setfont
  setmatrix
  moveto
}
%\def\pst@usecolor#1{\csname color@#1\endcsname\space}%    hv 1.14  2005--12-17
\def\pst@usecolor#1{\csname\string\color@#1\endcsname\space}
%
\def\newgray#1#2{%
  \pst@checknum{#2}\pst@tempg
  \@newcolor{#1}{\pst@tempg setgray}}
\def\newrgbcolor#1#2{%
  \pst@expandafter\pst@getnumiii{#2} {} {} {} {}\@nil
  \@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi setrgbcolor}}
\def\newhsbcolor#1#2{%
  \pst@expandafter\pst@getnumiii{#2} {} {} {} {}\@nil
  \@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi sethsbcolor}}
\def\newcmykcolor#1#2{%
  \pst@expandafter\pst@getnumiv{#2} {} {} {} {} {}\@nil
  \@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi \pst@tempj setcmykcolor}}
\newgray{black}{0}
\newgray{darkgray}{.25}
\newgray{gray}{.5}
\newgray{lightgray}{.75}
\newgray{white}{1}
\newrgbcolor{red}{1 0 0}
\newrgbcolor{green}{0 1 0}
\newrgbcolor{blue}{0 0 1}
\newrgbcolor{yellow}{1 1 0}
\newrgbcolor{cyan}{0 1 1}
\newrgbcolor{magenta}{1 0 1}
%
\define@key[psset]{pstricks}{bgcolor}{\def\pst@bgcolor{#1}}% background for pspicture
\psset[pstricks]{bgcolor={}}% \pst@bgcolor is \@empty

\define@key[psset]{pstricks}{style}{%
  \@ifundefined{pscs@#1}%
    {\@pstrickserr{Custom style `#1' undefined}\@ehpa}%
    {\@nameuse{pscs@#1}}%
}
\def\newpsstyle#1#2{\@namedef{pscs@#1}{%
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty\else\psset{#2}\fi}%
}
\def\addto@psstyle#1#2{%
    \pst@toks=\expandafter{#1#2}%
    \edef#1{\the\pst@toks}}
\def\addtopsstyle#1#2{%
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty\else
    \@ifundefined{pscs@#1}%
      {\newpsstyle{#1}{#2}}%
      {\expandafter\addto@psstyle\csname pscs@#1\endcsname{\psset{#2}}}%
  \fi}
%------------ hv 1.16 end -------------------
%
\def\@none{none}
\def\pst@getcolor#1#2{%
%  \@ifundefined{color@#1}%	hv 1.14  2005-12-17
  \@ifundefined{\string\color@#1}%
    {\@pstrickserr{Color `#1' not defined}\@eha}%
    {\edef#2{#1}}%
}
\newdimen\psunit \psunit 1cm
\newdimen\psxunit \psxunit 1cm
\newdimen\psyunit \psyunit 1cm
\let\psrunit\psunit
%
\def\pstunit@off{\let\@psunit\ignorespaces\ignorespaces}
%
\def\pssetlength#1#2{%
  \let\@psunit\psunit
  \afterassignment\pstunit@off
  #1 #2\@psunit%
}
\def\psaddtolength#1#2{%
  \let\@psunit\psunit
  \afterassignment\pstunit@off
  \advance#1 #2\@psunit%
}
\def\pssetxlength#1#2{%
  \let\@psunit\psxunit
  \afterassignment\pstunit@off
  #1 #2\@psunit%
}
\def\pssetylength#1#2{%
  \let\@psunit\psyunit
  \afterassignment\pstunit@off
  #1 #2\@psunit%
}
\define@key[psset]{pstricks}{unit}[1cm]{%
  \pssetlength\psunit{#1}%
  \psxunit=\psunit%
  \psyunit=\psunit%
}
\define@key[psset]{pstricks}{runit}[1cm]{\pssetlength\psrunit{#1}}
\define@key[psset]{pstricks}{xunit}[1cm]{\pssetxlength\psxunit{#1}}
\define@key[psset]{pstricks}{yunit}[1cm]{\pssetylength\psyunit{#1}}
%
\define@key[psset]{pstricks}{PstDebug}[0]{\pst@getint{#1}\Pst@Debug}% hv 2004-06-22
\psset[pstricks]{PstDebug=0}
\def\psDEBUG{\@ifnextchar[\psDEBUG@i{\psDEBUG@i[PSTricks]}}%
\def\psDEBUG@i[#1]#2{\ifnum\Pst@Debug>0 \expandafter\typeout{<#1>: #2}\fi}%
%
\def\pst@getlength#1#2{%
  \pssetlength\pst@dimg{#1}%
  \edef#2{\pst@number\pst@dimg}%
}
\def\pst@@getlength#1#2{%
  \pssetlength\pst@dimg{#1}%
  \edef#2{\number\pst@dimg sp}%
}
\def\pst@getcoor#1#2{\pst@@getcoor{#1}\let#2\pst@coor}
\def\pst@coor{0 0 }
%
\def\pst@getcoors#1#2{%
  \def\pst@aftercoors{\addto@pscode{#1 \pst@coors }#2}%
  \def\pst@coors{}%
  \pst@@getcoors%
}
\def\pst@@getcoors(#1){%
  \pst@@getcoor{#1}%
  \edef\pst@coors{\pst@coor\pst@coors}%
  \@ifnextchar({\pst@@getcoors}{\pst@aftercoors}%
}
%
\newcount\pst@C@@rType% 0: default cartesian coordinates and angles
%
\def\pst@getangle#1#2{\pst@@getangle{#1}\let#2\pst@angle}
\def\pst@angle{0 }
%
\def\cartesian@coor#1,#2,#3\@nil{%
  \pssetxlength\pst@dimg{#1}%
  \pssetylength\pst@dimh{#2}%
  \edef\pst@coor{\pst@number\pst@dimg \pst@number\pst@dimh}%
}
\def\NormalCoor{%
  \def\pst@@getcoor##1{\pst@expandafter\cartesian@coor{##1},\relax,\@nil}%
  \def\pstCheckCoorType##1{\global\pst@C@@rType=0}%
  \Pst@SpecialLengthfalse
  \def\pssetlength##1##2{%
    \let\@psunit\psunit
    \afterassignment\pstunit@off
    ##1 ##2\@psunit%
  }%
  \def\pst@@getangle##1{%
    \pst@checknum{##1}\pst@angle%
    \edef\pst@angle{\pst@angle \pst@angleunit}%
  }%
  \def\psput@##1{\pst@@getcoor{##1}\leavevmode\psput@cartesian}%
}
%\NormalCoor% set to normal read of coors, angles and lengths
%
\def\degrees{\@ifnextchar[{\@degrees}{\def\pst@angleunit{}}}
\def\@degrees[#1]{%
  \pst@checknum{#1}\pst@tempg
  \edef\pst@angleunit{360 \pst@tempg div mul }%
  \ignorespaces}
%
\def\radians{\def\pst@angleunit{57.2956 mul }}
\def\pst@angleunit{}
%
\def\SpecialCoor{%
  \def\pst@@getcoor##1{%
    \begingroup%
      \pst@activecoor%
      \xdef\pst@tempg{##1}%
    \endgroup%
    \expandafter\special@coor\pst@tempg||\@nil}%
  \def\pstCheckCoorType##1{%
    \begingroup%
      \pst@activecoor%
      \xdef\pst@tempg{##1}%
    \endgroup
    \psDEBUG[pstCheckCoorType]{:Checking coor \pst@tempg:}%
    \expandafter\pst@CheckCoorType\pst@tempg||\@nil%
    \psDEBUG[pstCheckCoorType]{::Coor type=\the\pst@C@@rType::}%
  }%
  \def\pssetlength##1##2{%
    \begingroup%
      \pst@activecoor%
      \xdef\pst@tempg{##2}%
    \endgroup%
    \expandafter\special@length\pst@tempg\@nil{##1}%
  \ignorespaces}%
  \def\pst@@getangle##1{%
    \begingroup%
      \pst@activecoor%
      \xdef\pst@tempg{##1}%
    \endgroup%
    \expandafter\special@angle\pst@tempg\@empty)\@nil%
  }%
  \def\psput@##1{\pst@@getcoor{##1}\leavevmode\psput@special}%
}
\SpecialCoor% set to special read of coors, angles and lengths
%
\define@key[psset]{}{precode}{\def\pst@prepscode{#1 }}
\define@key[psset]{}{postcode}{\def\pst@postpscode{#1 }}
\psset{precode={},postcode={}}% For use in other packages
%
%
\begingroup
\catcode`\|=13
\catcode`\;=13
\catcode`\!=13
\catcode`\*=13
\catcode`\>=13
\catcode`\+=13
\gdef\pst@activecoor{%
  \def|{\string|}%
  \def;{\string;}%
  \def!{\string!}%
  \def*{\string*}%			algebraic expression hv 2007-11-17
  \def>{\string>}%
  \def+{\string+}%			pure algebaric 2013-04-23
}
\endgroup
% \pst@C@@rType = 0 cartesian (x,y)
%               = 1 polar     (r;phi)
%               = 2 PS        (! x y)
%               = 3 mixed     ((x,y)|(x,y))
%               = 4 algebraic (*x f(x))   x in PostScript notation
%               = 5 node      (A)
%               = 6 special node ([...]A)
%               = 7 node      (>A)
%               = 8 algebraic (+x,f(x))   _both_ algebraic
\def\pst@CheckCoorType#1|#2|#3\@nil{%
  \ifx#3|\relax 
    \global\pst@C@@rType=3\relax
  \else 
    \expandafter\pst@@CheckCoorType#1;;\@nil%
  \fi}
%
\def\pst@@CheckCoorType#1#2;#3;#4\@nil{%
%\typeout{====1:#1}%
%\typeout{====2:#2}%
%\typeout{====3:#3}%
%\typeout{====4:#4}%
  \ifx#1>\relax%			node with special rotation for \uput
    \global\pst@C@@rType=7\relax%
  \else
    \ifcat#1a\relax%			node names should start with a letter
      \global\pst@C@@rType=5\relax%
    \else
      \ifx#1[\relax%			special node coor: [..]A
        \global\pst@C@@rType=6\relax%
      \else
        \ifx#1!\relax%			PostScript code: x y
          \global\pst@C@@rType=2\relax%
        \else
          \ifx#1*\relax%			algebraic PostScript code: x f(x)
            \global\pst@C@@rType=4\relax%
          \else
            \ifx#1+\relax%			algebraic algebraic: x, f(x)
              \global\pst@C@@rType=8\relax%
  	    \else
              \ifx#4;\relax%		polar coordinates
                \global\pst@C@@rType=1\relax%
              \else
                \global\pst@C@@rType=0\relax%
              \fi
            \fi
          \fi
	\fi
      \fi
    \fi
  \fi
  \psDEBUG[pstCheckCoorType]{::\the\pst@C@@rType::}%
  }%
%
%
\def\special@coor#1|#2|#3\@nil{%
  \ifx#3|\relax
    \mixed@coor{#1}{#2}%
  \else
    \special@@coor#1;;\@nil%
  \fi}
%
\def\special@@coor#1{%
  \ifcat#1a\relax%			node names should start with a letter
    \def\ps@next{\node@coor#1}%
  \else
    \ifx#1[\relax%			special node coor: [..]A
      \def\ps@next{\Node@coor[}%
    \else
      \ifx#1>\relax%			PostScript code: x y
        \def\ps@next{\special@@@@coor}%
    \else
      \ifx#1!\relax%			PostScript code: x y
        \def\ps@next{\raw@coor}%
      \else
        \ifx#1*\relax%			PostScript/algebraic code: x f(x)
          \def\ps@next{\alg@coor}%
        \else
          \ifx#1+\relax%		algebraic code: x,f(x)
            \def\ps@next{\algalg@coor}%
	  \else%
            \def\ps@next{\special@@@coor#1}%
          \fi%
	\fi%
      \fi%
    \fi\fi%
  \fi%
  \ps@next%
}
\def\special@@@coor#1;#2;#3\@nil{%
  \ifx#3;\relax
    \polar@coor{#1}{#2}%
  \else
    \cartesian@coor#1,\relax,\@nil
  \fi%
}
\def\special@@@@coor#1#2;#3;#4\@nil{%
  \def\ps@A{A}\def\ps@B{#1}%
  \ifcat\ps@A\ps@B\relax%
    \node@coor#1#2;;\@nil%
  \else%
    \cartesian@coor#1#2,\relax,\@nil
  \fi%
}
\def\mixed@coor#1#2{%
  \begingroup%
% DG/SR modification begin - Oct. 27, 1997 - Patch 6
%\specialcoor@ii#1;;\@nil
%\let\pst@tempa\pst@coor
%\specialcoor@ii#2;;\@nil
    \special@@coor#1;;\@nil%
    \let\pst@tempa\pst@coor%
    \special@@coor#2;;\@nil%
% DG/SR modification end
    \xdef\pst@tempg{\pst@tempa pop \pst@coor exch pop }%
  \endgroup%
  \let\pst@coor\pst@tempg%
}
%
\def\polar@coor#1#2{%
%  \pssetlength\pst@dimg{#1}%
  \pssetlength\pst@dimb{#1}%	hv 2007-10-16  g is already used in get@@angle
  \pst@@getangle{#2}%
%  \edef\pst@coor{\pst@number\pst@dimg \pst@angle \tx@PtoC}%  dito
  \edef\pst@coor{\pst@number\pst@dimb \pst@angle \tx@PtoC }%
}
%
\def\raw@coor{\@ifnextchar !\raw@@coor\raw@@@coor}
\def\raw@@coor!#1;#2\@nil{%		PostScript code without using \tx@ScreenCoor 
  \edef\pst@coor{#1 }}
\def\raw@@@coor#1;#2\@nil{%		PostScript code 
  \edef\pst@coor{ #1 \tx@ScreenCoor }}
%
\def\alg@coor{\@ifnextchar*{\alg@@coor}{\alg@@@@coor}}
\def\alg@@coor*#1;#2\@nil{\expandafter\alg@@@coor#1\@nil}
\def\alg@@@coor#1 #2\@nil{%			algebraic PostScript code 
%\typeout{Nummer1: #1}%
%\typeout{Nummer2: #2}%
  \edef\pst@coor{%
    /Func (#1) AlgParser cvx def    
    /y #2 def
    y Func exch \tx@ScreenCoor }}
%
\def\alg@@@@coor#1;#2\@nil{\expandafter\alg@@@@@coor#1\@nil}
\def\alg@@@@@coor#1 #2\@nil{%			algebraic PostScript code 
  \edef\pst@coor{%
    /x #1 def
    /Func (#2) AlgParser cvx def 
    x Func \tx@ScreenCoor }}
%
\define@boolkey[psset]{}[Pst@]{exchange}[true]{}
\psset{exchange=false}
%
\def\algalg@coor#1;#2\@nil{\expandafter\algalg@@@coor#1\@nil}
\def\algalg@@@coor#1,#2\@nil{%			algebraic algebraic code 
  \edef\pst@coor{%
    /x (#1) AlgParser cvx def    
    /Func (#2) AlgParser cvx def    
    x Func \tx@ScreenCoor  }}
%
\def\node@coor#1\@nil{%
  \@pstrickserr{You must load `pst-node.tex' to use node coordinates.}\@ehps
  \def\pst@coor{0 0 }%
}
\def\Node@coor{\node@coor}
%
\def\special@angle#1#2)#3\@nil{%
  \ifx !#1\relax
    \edef\pst@angle{#2\space \pst@angleunit}%
  \else\ifx(#1\relax
    \pst@@getcoor{#2}%
    \edef\pst@angle{\pst@coor exch \tx@Atan}%
  \else
    \pst@checknum{#1#2}\pst@angle
    \edef\pst@angle{\pst@angle \pst@angleunit}%
  \fi\fi}
%
\def\special@length#1#2\@nil#3{%
  \psDEBUG[special@length]{ #1|#2|#3 }%
  \ifx !#1\relax
    \edef\pst@SpecialLength{ #2 \pst@number\psunit mul }%
    \Pst@SpecialLengthtrue%
    \psDEBUG[special@length]{ Special length: \pst@SpecialLength}%
  \else
    \let\@psunit\psunit
    \afterassignment\pstunit@off
    #3 #1#2\@psunit%
    \Pst@SpecialLengthfalse%
  \psDEBUG[special@length]{ Normal length: \the#3 }%
  \fi}
%
\def\Cartesian{%
  \def\cartesian@coor##1,##2,##3\@nil{%
    \pssetxlength\pst@dimg{##1}%
    \pssetylength\pst@dimh{##2}%
    \edef\pst@coor{\pst@number\pst@dimg \pst@number\pst@dimh}%
  }%
  \@ifnextchar({\Cartesian@}{}%
}
\def\Cartesian@(#1,#2){%
  \pssetxlength\psxunit{#1}%
  \pssetylength\psyunit{#2}%
  \ignorespaces%
}
\def\Polar{%
  \def\psput@cartesian{\psput@special}%
  \def\cartesian@coor##1,##2,##3\@nil{\polar@coor{##1}{##2}}%
}%
\define@key[psset]{pstricks}{origin}[]{%
  \pst@@getcoor{#1}%
  \edef\psk@origin{\pst@coor T }}
\def\psk@origin{}
%
\define@boolkey[psset]{pstricks}[Pst@]{algebraic}[true]{}
\psset%[pstricks]
{algebraic=false}
%
\define@boolkey[psset]{pstricks}[]{swapaxes}[true]{%			\if@pst
  \@nameuse{@pst#1}%
  \if@pst\def\psk@swapaxes{-90 rotate -1 1 scale }%
  \else\def\psk@swapaxes{}%
  \fi}
\psset[pstricks]{swapaxes=false}
%
\define@boolkey[psset]{pstricks}[]{showpoints}[true]{}
\psset[pstricks]{showpoints=false}
%
\let\pst@setrepeatarrowsflag\relax
%
\define@key[psset]{pstricks}{border}[0pt]{\pst@getlength{#1}\psk@border \pst@setrepeatarrowsflag}
\psset[pstricks]{border=0pt}
\define@key[psset]{pstricks}{bordercolor}[white]{\pst@getcolor{#1}\psbordercolor}
\psset[pstricks]{bordercolor=white}
\define@boolkey[psset]{pstricks}[ps]{doubleline}[true]{\pst@setrepeatarrowsflag}
\psset[pstricks]{doubleline=false}
\define@key[psset]{pstricks}{doublesep}[1.25\pslinewidth]{\def\psdoublesep{#1}}
\psset[pstricks]{doublesep=1.25\pslinewidth}
\define@key[psset]{pstricks}{doublecolor}[white]{\pst@getcolor{#1}\psdoublecolor}
\psset[pstricks]{doublecolor=white}
%
\define@boolkey[psset]{pstricks}[ps]{shadow}[true]{\pst@setrepeatarrowsflag}
\psset[pstricks]{shadow=false}
\define@key[psset]{pstricks}{shadowsize}[3pt]{\pst@getlength{#1}\psk@shadowsize}
\psset[pstricks]{shadowsize=3pt}
\define@key[psset]{pstricks}{shadowangle}[-45]{\pst@getangle{#1}\psk@shadowangle}
\psset[pstricks]{shadowangle=-45}
\define@key[psset]{pstricks}{shadowcolor}[darkgrey]{\pst@getcolor{#1}\psshadowcolor}
\psset[pstricks]{shadowcolor=darkgray}
%
\def\pst@repeatarrowsflag{\z@}
\def\pst@setrepeatarrowsflag{%
  \edef\pst@repeatarrowsflag{%
    \ifdim\psk@border\p@>\z@ 1\else\ifpsdoubleline 1\else
      \ifpsshadow 1\else \z@\fi\fi\fi}}
%
\def\psls@none{}
\def\psls@solid{ \psk@linejoin\space setlinejoin \psk@linecap\space setlinecap stroke }
\def\psls@coloreddashed{ \psls@solid grestore gsave \pst@usecolor\psdashcolor \tx@setlinejoin \psls@dashed }
%
\newdimen\pslinewidth
\define@key[psset]{pstricks}{linewidth}[0.8pt]{\pssetlength\pslinewidth{#1}}
\psset[pstricks]{linewidth=.8pt}
\define@key[psset]{pstricks}{linecolor}[black]{\pst@getcolor{#1}\pslinecolor}
\psset[pstricks]{linecolor=black}
\define@key[psset]{pstricks}{kitecolor}[red]{\pst@getcolor{#1}\ps@kitecolor}
\define@key[psset]{pstricks}{dartcolor}[blue]{\pst@getcolor{#1}\ps@dartcolor}
\psset[pstricks]{kitecolor,dartcolor}
%
\newif\ifPst@coloreddashed
\define@key[psset]{pstricks}{dashcolor}[white]{%
  \ifx\relax#1\relax\Pst@coloreddashedfalse%
  \else\Pst@coloreddashedtrue\pst@getcolor{#1}\psdashcolor
  \fi}
\psset{dashcolor=\relax}
%\define@key[psset]{pstricks}{linecap}[0]{\pst@getint{#1}\psk@linecap}%	hv 2007-12-01
%\psset[pstricks]{linecap=0}  >>>>>>>>>>>>> siehe unten
\define@key[psset]{pstricks}{linejoin}[0]{\pst@getint{#1}\psk@linejoin}%	hv 2007-10-13
\psset[pstricks]{linejoin=0}
\def\tx@setlinejoin{\psk@linejoin\space setlinejoin }%	hv 2007-10-13
%
\def\pst@missing{%
  \z@
  \@pstrickserr{Missing number or dimension. 0 substituted}\@ehpa}
%
%%------------------- begin patch 15 HV 2004-05-15 -------------
\def\pst@empty{\z@}

\define@key[psset]{pstricks}{dash}[5pt 3pt 0pt 0pt]{%	defined in pstricks.tex
  \pst@expandafter\psset@@dash{#1}\@nil}% Error handling for empty argument.
\define@key[psset]{pstricks}{maxdashes}[11]{\def\psk@maxdashes{#1}}
\psset[pstricks]{maxdashes=11}
%
\def\psset@@dash#1\@nil{%
 \def\psk@dash{}%
 \pst@cntm0
 \def\next##1 ##2\relax{%
   \expandafter\ifnum\psk@maxdashes>\pst@cntm\relax  % 04-08-07
     \edef\@tempa{##1}%
     \ifx\@tempa\@empty\else% gobble leading spaces
       \pssetlength\pst@dimc{##1}%
       \advance\pst@cntm by 1
       \edef\psk@dash{\psk@dash\space\pst@number\pst@dimc}%
     \fi%
     \edef\@tempa{##2}%
     \ifx\@tempa\@empty\else% detect end
       \ifx\@tempa\space\else% gobble trailing spaces
         \next##2\relax%
     \fi\fi%
   \else% 04-08-07
     \@pstrickserr{Number of dashes > \psk@maxdashes. Increasing 
        'maxdashes' might work.}\@ehpa% 04-08-07
   \fi% 04-08-07
 }%
 \expandafter\next#1 \relax}
\psset[pstricks]{dash=5pt 3pt 0pt 0pt}% black white black white 
%%------------------- end patch 15 HV 2004-05-15 -------------
\define@boolkey[psset]{pstricks}[ps]{dashadjust}[true]{}
\psset[pstricks]{dashadjust}
\def\tx@DashLine{DashLine }
%
\def\psls@dashed{
  \ifPst@coloreddashed \psls@solid grestore gsave \pst@usecolor\psdashcolor \tx@setlinejoin \fi
  \psk@linecap\space setlinecap 
  \ifpsdashadjust
    [ \psk@dash ] \pst@linetype\space \tx@DashLine
  \else
    [ \psk@dash ] 0 setdash stroke
  \fi}
%% End patch TN; Date (YY-MM-DD): 04-07-17; 2nd part
%
\define@key[psset]{pstricks}{dotsep}[3pt]{\pst@getlength{#1}\psk@dotsep}
\psset[pstricks]{dotsep=3pt}
\def\tx@DotLine{DotLine }
\def\psls@dotted{
  \ifpsdashadjust
    \psk@dotsep \pst@linetype\space \tx@DotLine
  \else
    [ 0 \psk@dotsep CLW add ] 0 setdash 1 setlinecap stroke
  \fi
}
%
\define@key[psset]{pstricks}{linestyle}[solid]{%
  \@ifundefined{psls@#1}%
    {\@pstrickserr{Line style `#1' not defined}\@eha}%
    {\def\pslinestyle{#1}}}
\psset[pstricks]{linestyle=solid}
%
\define@key[psset]{pstricks}{linecap}[0]{%
  \def\psk@linecap{0}%
  \ifnum#1>-1
    \ifnum#1<3
      \pst@getint{#1}\psk@linecap%
  \fi\fi}
\psset{linecap=0}
%------------------------- Transparency modes ----------------------------
\pst@def{setTransparency}< \psk@opacityalpha .setopacityalpha >
\pst@def{setStrokeTransparency}< \psk@strokeopacityalpha .setopacityalpha >
\pst@def{setBlendmode}<
    \ifcase\psk@blendmode
      /Normal \or
      /Compatible \or
      /Screen \or
      /Multiply \or
      /HardLight \or
      /Darken \or
      /Lighten \or
      /Difference\or
      /ColorDodge\or
      /ColorBurn\or
      /SoftLight\or
      /Hue\or
      /Saturation\or
      /Luminosity\or
      /Overlay\or
      /Exclusion\or
      /Color
    \else
      /Normal 
    \fi
    .setblendmode \psk@shapealpha .setshapealpha >
%
%--------------------------------- hv 2007-09-09 begin ---------------------
% transparency needs a run through latex -> dvips -> ps2pdf14(!) 
%
\def\e@fill@inverse{oefill}
\define@key[psset]{pstricks}{fillcolor}[white]{%
  \ifx\psk@fillstylename\e@fill@inverse
    \pst@getcolor{#1}\psk@oefillcolor
    \pst@getcolor{white}\psfillcolor
  \else \pst@getcolor{white}\psk@oefillcolor
        \pst@getcolor{#1}\psfillcolor
  \fi}

\psset[pstricks]{fillcolor=white}
\define@key[psset]{pstricks}{strokeopacity}[1]{\pst@checknum{#1}\psk@strokeopacityalpha }% for lines
\psset[pstricks]{strokeopacity=1}
\define@key[psset]{pstricks}{opacity}[1]{\pst@checknum{#1}\psk@opacityalpha }% for filled areas 
\psset[pstricks]{opacity=1}
\define@key[psset]{pstricks}{shapealpha}[0.6]{\pst@checknum{#1}\psk@shapealpha }
\psset[pstricks]{shapealpha=0.6}
\define@key[psset]{pstricks}{blendmode}[0]{\pst@getint{#1}\psk@blendmode }% must be one of 
% /Normal     0
% /Compatible 1
% /Screen     2
% /Multiply   3
% /HardLight  4
\psset[pstricks]{blendmode=0}
\define@key[psset]{pstricks}{fsAngle}[137.50775]{\pst@getangle{#1}\pst@fsAngle }
\define@key[psset]{pstricks}{fsOrigin}[(0,0)]{%
  \pst@@getcoor{#1}\edef\pst@fsOrigin{\pst@coor T }}
\psset[pstricks]{fsOrigin={0,0},fsAngle=137.50775}
%
\def\tx@LineFill{LineFill }
\def\tx@DotFill{DotFill }
\def\tx@PenroseFill{PenroseFill }
\def\tx@PenroseFillA{PenroseFillA }
\def\tx@TruchetFill{TruchetFill }
%
\def\psfs@none{}
\def\psfs@solid{\pst@fill{\pst@usecolor\psfillcolor \tx@setTransparency fill }}
\def\psfs@eofill{\pst@fill{\pst@usecolor\psfillcolor \tx@setTransparency eofill}}
\def\psfs@oefill{\pst@fill{\pst@usecolor\psk@oefillcolor  \tx@setTransparency fill } \psfs@eofill }
\def\psfs@shape{\pst@fill{\pst@usecolor\psfillcolor \tx@setBlendmode fill }}
\def\psfs@spiral{\pst@fill{\pst@fsOrigin \pst@usecolor\psfillcolor clip newpath
    0 .1 500 { dup dup sqrt 4 div 0 360 arc fill \pst@fsAngle rotate } for }}
%
\define@key[psset]{pstricks}{hatchwidth}[0.8pt]{\pst@getlength{#1}\psk@hatchwidth}
\psset[pstricks]{hatchwidth=.8pt}
\define@key[psset]{pstricks}{hatchsep}[4pt]{\pst@getlength{#1}\psk@hatchsep}
\psset[pstricks]{hatchsep=4pt}
\define@key[psset]{pstricks}{hatchcolor}[black]{\pst@getcolor{#1}\pshatchcolor}
\psset[pstricks]{hatchcolor=black}
\define@key[psset]{pstricks}{hatchangle}[45]{\pst@getangle{#1}\psk@hatchangle}
\psset[pstricks]{hatchangle=45}
\define@key[psset]{pstricks}{hatchsepinc}[0pt]{\pst@getlength{#1}\psk@hatchsepinc}
\define@key[psset]{pstricks}{hatchwidthinc}[0pt]{\pst@getlength{#1}\psk@hatchwidthinc}
\psset[pstricks]{hatchwidthinc=0pt,hatchsepinc=0pt}
%
\def\pst@linefill#1{
  /clipType { \ifx\relax#1\relax clip \else#1\fi} def 
  \psk@hatchangle rotate
  \psk@hatchwidth SLW
  \pst@usecolor\pshatchcolor
  \psk@hatchsep 
  \psk@hatchsepinc
  \psk@hatchwidthinc
  \tx@LineFill }
%
\def\psfs@vlines{\pst@fill{\pst@linefill{}}}
\def\psfs@eovlines{\pst@fill{\pst@linefill{eoclip}}}
\@namedef{psfs@vlines*}{\psfs@solid \psfs@vlines}
\@namedef{psfs@eovlines*}{\psfs@eofill \psfs@eovlines}
\def\psfs@hlines{\pst@fill{90 rotate \pst@linefill{}}}
\def\psfs@eohlines{\pst@fill{90 rotate \pst@linefill{eoclip}}}
\@namedef{psfs@hlines*}{\psfs@solid \psfs@hlines}
\@namedef{psfs@eohlines*}{\psfs@eofill \psfs@eohlines}
\def\psfs@crosshatch{\psfs@vlines \psfs@hlines}
\@namedef{psfs@crosshatch*}{\psfs@solid \psfs@vlines \psfs@hlines}
\@namedef{psfs@eocrosshatch*}{\psfs@eofill \psfs@eovlines \psfs@eohlines}
%
\define@key[psset]{pstricks}{psscale}[1]{%
  \def\psk@@psscale{#1}%   for use with \psscalebox
  \pst@checknum{#1}\psk@psscale}
\psset[pstricks]{psscale=1}
%
\def\pst@dotFill[#1]{%
  /clipType { \ifx\relax#1\relax clip \else #1 \fi } def 
  gsave
  \pst@number\pslinewidth SLW
  \pst@usecolor\pshatchcolor
%  /DotLineColor { \pst@usecolor\pslinecolor } def
  \psk@hatchsep 
  \psk@hatchwidth
  \tx@DotFill }

\def\psfs@dots{\pst@fill{ /SolidDot false def \pst@dotFill[] }}
\def\psfs@eodots{\pst@fill{ /SolidDot false def \pst@dotFill[eoclip] }}
\@namedef{psfs@dots*}{\pst@fill{ /SolidDot true def \pst@dotFill[] }}
\@namedef{psfs@eodots*}{\pst@fill{ /SolidDot true def \pst@dotFill[eoclip] }}
%
\def\pst@penroseFill{%
%  gsave					% restore in PenroseFill
  \pst@number\pslinewidth SLW
  \pst@usecolor\pshatchcolor
  \psk@psscale 
  \tx@PenroseFill }
\def\psfs@penrose{\pst@fill\pst@penroseFill}
\@namedef{psfs@penrose*}{\psfs@solid \psfs@penrose}
%
\def\pst@penroseFillA{%
%  gsave					% restore in PenroseFillA
  \pst@number\pslinewidth SLW
%  \pst@usecolor\pshatchcolor
%  on stack: scaling factor, border color, kite color, dart color
%  dup dup scale
%  /border_colour ED % 
%  /kite_colour ED %
%  /dart_colour 
  { \pst@usecolor\ps@dartcolor }
  { \pst@usecolor\ps@kitecolor }
  { \pst@usecolor\pshatchcolor }
  \psk@psscale 
  \tx@PenroseFillA }
\def\psfs@penroseA{\pst@fill\pst@penroseFillA}
\@namedef{psfs@penroseA*}{\psfs@solid \psfs@penroseA}
%
\def\pst@truchetFill{%
  gsave					% restore in PenroseFill
  \pst@number\pslinewidth SLW
  \pst@usecolor\pshatchcolor
  \psk@psscale 
  \tx@TruchetFill }
\def\psfs@truchet{ \pst@fill\pst@truchetFill }
\@namedef{psfs@truchet*}{\psfs@solid \psfs@truchet}
%
\define@key[psset]{pstricks}{fillstyle}[none]{%
  \def\psk@fillstylename{#1}%  needed for inverse eofill
  \edef\pst@tempg{#1}\def\pst@temph{none}%
  \ifx\pst@tempg\pst@temph
     \let\psk@fillstyle\relax
  \else
    \@ifundefined{psfs@#1}%
    {\@pstrickserr{Undefined fill style: `#1'}\@eha}%
    {\edef\psk@fillstyle{\expandafter\noexpand\csname psfs@#1\endcsname}}%
  \fi%
}
\define@key[psset]{pstricks}{addfillstyle}[]{%
  \@ifundefined{psfs@#1}%
    {\@pstrickserr{Undefined fill style: `#1'}\@eha}%
    {\edef\psk@fillstyle{%
      \expandafter\noexpand\psk@fillstyle
      \expandafter\noexpand\csname psfs@#1\endcsname}%
    }}
\psset[pstricks]{fillstyle=none}
%
%--------------------------- continous linewidth -------------------
\newdimen\psk@startLW
\newdimen\psk@endLW
\define@key[psset]{pstricks}{startLW}[\pslinewidth]{\pssetlength{\psk@startLW}{#1}}%
\define@key[psset]{pstricks}{endLW}[\pslinewidth]{\pssetlength{\psk@endLW}{#1}}%
\define@key[psset]{pstricks}{startWL}[380]{\pst@getint{#1}\psk@startWL}%
\define@key[psset]{pstricks}{endWL}[780]{\pst@getint{#1}\psk@endWL}%
\define@boolkey[psset]{pstricks}[Pst@]{variableLW}[true]{}
\define@boolkey[psset]{pstricks}[Pst@]{variableColor}[true]{}
\define@key[psset]{pstricks}{setflat}[0.1]{\pst@checknum{#1}\psk@setflat}%
\psset[pstricks]{startLW=\pslinewidth,endLW=\pslinewidth,variableColor=false,
  variableLW=false,startWL=380,endWL=780,setflat=0.1}
%
\def\pst@flattenpath{
  /Coors [] def         % the array of all points
  /lambda \psk@startWL\space def
  %
  /add2Values { Coors aload length 2 add array astore /Coors exch def } def
  /add6Values { Coors aload length 6 add array astore /Coors exch def } def
%
  \psk@setflat\space setflat   % the value for the line snippets
  flattenpath            % flatten the existing path into line segments
%
  { add2Values }         % what to do with moveto
  { add2Values }         % what to do with lineto 
  { add6Values }         % what to do with curveto (not needed here) 
  { }                    % what to do with closepath
  pathforall             % do it for the existing path
%
  \pst@number\psk@startLW setlinewidth
  \tx@setlinejoin
  \psk@linecap\space setlinecap
  Coors aload length 2 sub 2 div cvi /N0 exch def % set number of points
  /NN 0 def
  /N N0 def
  { N 3 gt { N 3 sub /N ED }{ N 1 sub /N ED } ifelse 
    NN 1 add /NN ED
    N 0 eq { exit } if
  } loop
  /dLW \pst@number\psk@endLW \pst@number\psk@startLW sub NN div def          % the step for the linewidth
  \ifPst@variableColor
    /dColor \psk@endWL\space \psk@startWL\space sub NN div def
    lambda dColor add dup /lambda ED 
    tx@addDict begin wavelengthToRGB Red Green Blue end setrgbcolor
  \else
    \pst@usecolor\pslinecolor
  \fi
  moveto                 % move to the first one
  /N N0 def
  {
    N 3 gt {  
%    CP 6 2 roll
    \psk@curvature\space /c ED /b ED /a ED
    /ArrowA {} def
    /ArrowB {} def
    BOC NC EOC %    curveto 
    N 3 sub /N ED }{ lineto N 1 sub /N ED } ifelse
    currentlinewidth dLW add setlinewidth % increase line width
    \ifPst@variableColor
      lambda dColor add dup /lambda ED 
      tx@addDict begin wavelengthToRGB Red Green Blue end setrgbcolor
    \else
      \pst@usecolor\pslinecolor
    \fi
    CP /Y ED /X ED       % put coors of current point on the stack
%    0.4 .setopacityalpha 
    stroke               % draw the line segment
    N 0 eq { exit }{ X Y moveto } ifelse
  } loop
%  N {                    % repeat for the other N coords
%    lineto               % line to next point
%    currentlinewidth dLW add setlinewidth % increase line width
%    lambda dColor add dup /lambda ED 
%    tx@addDict begin wavelengthToRGB Red Green Blue end setrgbcolor
%    currentpoint         % put coors of current point on the stack
%    0.4 .setopacityalpha 
%    stroke               % draw the line segment
%    moveto
%  } repeat
}

%
%--------------------------- A R R O W S ---------------------------
%
\def\psk@arrowA{}
\def\psk@arrowB{}
\def\pst@arrowtable{,-,<->,<<->>,>-<,>>-<<,(-),[-],)-(,]-[,|>-<|,<D-D>,D>-<D,<D<D-D>D>} % hv --1.16
\edef\pst@arrowtable{\pst@arrowtable,|<*->|*,|<->|}
\begingroup
  \catcode`\<=13
  \catcode`\>=13
  \catcode`\|=13
  \gdef\pst@activearrows{\def<{\string<}\def>{\string>}\def|{\string|}}
\endgroup
\def\tx@BeginArrow{BeginArrow }
\def\tx@EndArrow{EndArrow }
%
\def\tx@Arrow{ \tx@setStrokeTransparency Arrow }% hv 2008-01-13
\def\tx@ArrowD{ \tx@setStrokeTransparency ArrowD }% hv 2008-01-13
%
\@namedef{psas@<|}{ 
    \psk@tbarsize\space \tx@Tbar
    0 CLW 2 div T
    newpath
    true 
    \psk@arrowinset 
    \psk@arrowlength 
    \psk@arrowsize 
    \tx@Arrow 
}
% ]-[ arrow
\def\tx@BracketOut{BracketOut }
\@namedef{psas@[}{%
  /BracketOut {%
  CLW mul add dup CLW sub 2 div
%/x ED mul CLW add
  /x ED mul neg
  /y ED
  /z CLW 2 div def
  x neg y moveto
  x neg CLW 2 div L x CLW 2 div L x y L stroke 0 CLW moveto } def
  \psk@bracketlength\space \psk@tbarsize\space \tx@BracketOut
}
% )-( arrow
\def\tx@RoundBracketOut{ \tx@setStrokeTransparency RoundBracketOut }% hv 2008-01-13
\@namedef{psas@(}{%
  /RoundBracketOut {%
    CLW mul add dup 2 div
%/x ED mul
    /x ED mul neg
    /y ED
    /mtrx CM def
    0 CLW
    2 div T x y mul 0 ne { x y scale } if
    1 1 moveto
    .85 .5 .35 0 0 0 curveto
    -.35 0 -.85 .5 -1 1 curveto
    mtrx setmatrix stroke 0 CLW moveto } def
  \psk@rbracketlength\space \psk@tbarsize\space \tx@RoundBracketOut
}
% end of new definitions of the missing arrows ---- hv 1.12
\@namedef{psas@>}{ false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow }
\@namedef{psas@>>}{%
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
  0 h T gsave newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
  CP grestore CP newpath moveto 2 copy 
  CLW \pst@arrowscale\space div SLW % set the original line width  
  L stroke moveto
}
\@namedef{psas@<}{true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow}
\@namedef{psas@<<}{
  true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
  CP newpath moveto 0 a neg 
  gsave
  CLW \pst@arrowscale\space div SLW % set the original line width  
  L stroke 
  grestore
  0 h neg T
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
}
\@namedef{psas@D>}{ false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD }%	hv 20071211
\@namedef{psas@D>D>}{ %	hv 20071211
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD
  0 h Inset sub T gsave newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD
  CP grestore moveto 
}
\@namedef{psas@<D}{ %	hv 20071211
  true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD
}
\@namedef{psas@<D<D}{ %	hv 20071211
  true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD
  CP newpath moveto 0 a neg L stroke 0 h neg T
  true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD
}
\define@key[psset]{pstricks}{tbarsize}[2pt 5]{%
  \pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil
  \edef\psk@tbarsize{\pst@number\pst@dimg \pst@tempg}}
\psset[pstricks]{tbarsize=2pt 5}
%
\def\tx@Tbar{Tbar }
\@namedef{psas@|}{\psk@tbarsize \tx@Tbar}
\@namedef{psas@|*}{0 CLW -2 div T \psk@tbarsize \tx@Tbar}
\@namedef{psas@>|}{%
  \psk@tbarsize \tx@Tbar
  0 CLW 2 div T
  newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
}
\@namedef{psas@>|*}{%
  0 CLW -2 div T
  \psk@tbarsize \tx@Tbar
  0 CLW 2 div T
  newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
}
%
\define@key[psset]{pstricks}{bracketlength}[0.15]{\pst@checknum{#1}\psk@bracketlength}
\psset[pstricks]{bracketlength=.15}
\def\tx@Bracket{Bracket }
\@namedef{psas@]}{\psk@bracketlength \psk@tbarsize \tx@Bracket}
\define@key[psset]{pstricks}{rbracketlength}[0.15]{\pst@checknum{#1}\psk@rbracketlength}
\psset[pstricks]{rbracketlength=.15}
\def\tx@RoundBracket{RoundBracket }
\@namedef{psas@)}{\psk@rbracketlength \psk@tbarsize \tx@RoundBracket}
%
\def\psas@c{1 \psas@@c}
\def\psas@cc{0 CLW 2 div T 1 \psas@@c}
\def\psas@C{2 \psas@@c}
\def\psas@@c{%
  setlinecap
  0 0 moveto
  0 0.1 L % changed value from 0.5 to 0.1
  stroke
  0 0 moveto }
%
\def\psas@{}
%
\define@key[psset]{pstricks}{arrowLW}{\pst@getlength{#1}\psk@arrowLW}
\psset[pstricks]{arrowLW=0}
% arrowLW as LineWidth for the circled line ends
%
\def\psas@o{\psk@arrowLW\space dup 0 eq { pop }{ SLW } ifelse
  {\pst@usecolor\psfillcolor true} false \psk@dotsize \tx@EndDot }
\def\psas@oo{\psk@arrowLW\space dup 0 eq { pop }{ SLW } ifelse
  {\pst@usecolor\psfillcolor true} true \psk@dotsize \tx@EndDot }
\@namedef{psas@*}{\psk@arrowLW\space dup 0 eq { pop }{ SLW } ifelse
  {false} false \psk@dotsize \tx@EndDot }
\@namedef{psas@**}{\psk@arrowLW\space dup 0 eq { pop }{ SLW } ifelse
  {false} true \psk@dotsize \tx@EndDot }
%
\define@key[psset]{pstricks}{arrows}[-]{%
  \begingroup
    \pst@activearrows
    \xdef\pst@tempg{#1}%
  \endgroup
  \expandafter\psset@@arrows\pst@tempg\@empty-\@empty\@nil
  \if@pst\else\@pstrickserr{Bad arrows specification: #1}\@ehpa\fi}
\def\psset@@arrows#1-#2\@empty#3\@nil{%
  \@psttrue
  \def\ps@next##1,#1-##2,##3\@nil{\def\pst@tempg{##2}}%
  \expandafter\ps@next\pst@arrowtable,#1-#1,\@nil
  \@ifundefined{psas@\pst@tempg}{\@pstfalse\def\psk@arrowA{}}{\let\psk@arrowA\pst@tempg}%
  \@ifundefined{psas@#2}{\@pstfalse\def\psk@arrowB{}}{\def\psk@arrowB{#2}}}
\psset[pstricks]{arrows=-}
%
\define@key[psset]{pstricks}{arrowscale}[1]{%                                   hv --1.12
  \pst@getscale{#1}\psk@arrowscale
  \pst@@arrowscale@i#1 \@nil}%           hv --1.12
\def\pst@@arrowscale@i#1 #2\@nil{\edef\pst@arrowscale{#1}}% hv --1.12
\psset[pstricks]{arrowscale=1}
%
\define@key[psset]{pstricks}{arrowsize}[1.5pt 2]{%
  \pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil
  \edef\psk@arrowsize{\pst@number\pst@dimg \pst@tempg}%
}
\psset[pstricks]{arrowsize=1.5pt 2}
\define@key[psset]{pstricks}{arrowlength}[1.4]{\pst@checknum{#1}\psk@arrowlength}
\psset[pstricks]{arrowlength=1.4}
\define@key[psset]{pstricks}{arrowinset}[0.4]{\pst@checknum{#1}\psk@arrowinset}%
\psset[pstricks]{arrowinset=0.4}
%
\def\tx@SD{ \tx@setTransparency SD }
\def\tx@EndDot{EndDot }
%
\def\pst@par{}
\def\addto@par#1{%
  \ifx\pst@par\@empty
    \def\pst@par{#1}%
  \else
    \expandafter\def\expandafter\pst@par\expandafter{\pst@par,#1}%
  \fi%
}
\def\addbefore@par#1{%
  \ifx\pst@par\@empty
    \def\pst@par{#1}%
  \else
    \toks@{#1}%
    \pst@toks\expandafter{\pst@par}%
    \edef\pst@par{\the\toks@,\the\pst@toks}%
  \fi%
}
\def\use@par{%
  \ifx\pst@par\@empty\else%
    \expandafter\@psset\pst@par,\@nil%
    \def\pst@par{}%
  \fi}
\def\use@keep@par{%			same as \use@par, but keeps the values
  \ifx\pst@par\@empty\else
    \expandafter\@psset\pst@par,\@nil
%    \def\pst@par{}%
  \fi}
%
\def\pst@object#1{%
  \def\pst@par{}%
  \pst@ifstar{%
    \@ifnextchar[{\pst@@object{#1}}{\@nameuse{#1@i}}}%
}
\def\pst@@object#1[#2]{%
  \def\pst@par{#2}%
  \@ifnextchar+{\@nameuse{#1@i}}{\@nameuse{#1@i}}%
}
\def\newpsobject#1#2#3{%
\@ifundefined{#2@i}%
{\@pstrickserr{Graphics object `#2' not defined}\@eha}{%
\@namedef{#1}{\pst@object{#1}}%
\@namedef{#1@i}{\addbefore@par{#3}\@nameuse{#2@i}}}%
\ignorespaces}
%
\def\pst@getarrows#1{\@ifnextchar({#1}{\pst@@getarrows{#1}}}
% ------------------------- hv 1.10 beg ------------------------
%\def\pst@@getarrows#1#2{\addto@par{arrows=#2}#1}
\def\pst@@getarrows#1#2{%
  \def\pst@tempa{#2}% prevent empty arrow arguments, to allow \psline{}(...)(...)
  \ifx\pst@tempa\@empty\addto@par{arrows=-}\else\addto@par{arrows=#2}\fi#1}
% ------------------------- hv 1.10 end ------------------------
%
\def\begin@ClosedObj{%
  \leavevmode%
  \pst@killglue%
  \begingroup%
  \use@par%
  \solid@star%
  \ifpsdoubleline\pst@setdoublesep\fi%
  \pst@addarrowdef% DG addition
  \init@pscode}
%
\def\end@ClosedObj{%
  \ifpsshadow \pst@closedshadow \fi
  \ifdim\psk@border\p@>\z@ \pst@addborder \fi
  \psk@fillstyle
  \pst@stroke
  \ifpsdoubleline \pst@doublestroke \fi
  \ifshowpoints
% DG modification begin - Mar. 4, 1995
%\addto@pscode{Points aload length 2 div cvi /N ED \psdots@iii}%
  \pst@OpenShowPoints
% DG modification end
  \fi
  \use@pscode
  \endgroup
  \ignorespaces%
}
\def\begin@OpenObj{%
  \begin@ClosedObj%
  \let\pst@linetype\pst@arrowtype%
  \pst@addarrowdef%
}
\def\begin@AltOpenObj{%
  \begin@ClosedObj
  \def\pst@repeatarrowsflag{\z@}%
  \def\pst@linetype{0}}
%
\def\end@OpenObj{%
  \ifpsshadow \pst@openshadow \fi
  \ifdim\psk@border\p@>\z@ \pst@addborder \fi
  \psk@fillstyle
  \pst@stroke
  \ifpsdoubleline \pst@doublestroke \fi
  \ifnum\pst@repeatarrowsflag>\z@ \pst@repeatarrows \fi
  \ifshowpoints \pst@OpenShowPoints \fi
  \use@pscode
  \endgroup
  \ignorespaces}
%
\def\begin@SpecialObj{%
  \leavevmode
  \pst@killglue
  \begingroup
  \use@par
  \init@pscode}
%
\def\end@SpecialObj{%
  \use@pscode
  \endgroup
  \ignorespaces}
%
\def\pst@code{}%
\def\init@pscode{%
  \addto@pscode{%
    \pst@number\pslinewidth SLW
    \pst@usecolor\pslinecolor}%
}
\def\addto@pscode#1{\xdef\pst@code{\pst@code#1\space}}
\def\use@pscode{%
  \pstverb{
    \pst@dict
    \tx@STP
    \pst@newpath
    \psk@origin
    \psk@swapaxes
    \pst@code
    end
  }%
  \gdef\pst@code{}%
}
\def\use@psCode{%
  \pstVerb{
    \pst@dict
    \tx@STP
    \pst@newpath
    \psk@origin
    \psk@swapaxes
    \pst@code
    end
  }%
  \gdef\pst@code{}%
}
\def\pst@newpath{newpath }
%
\def\pst@@killglue{\unskip\ifdim\lastskip>\z@\expandafter\pst@@killglue\fi}
\def\KillGlue{\let\pst@killglue\pst@@killglue}
\def\DontKillGlue{\let\pst@killglue\relax}
\DontKillGlue
%
\def\solid@star{%
  \if@star
    \pslinewidth=\z@
    \psdoublelinefalse
    \def\pslinestyle{none}%
    \def\psk@fillstyle{\psfs@solid}%
    \let\psfillcolor\pslinecolor
  \fi}
%
\def\pst@setdoublesep{%
\pst@getlength\psdoublesep\psdoublesep
\pslinewidth=2\pslinewidth
\advance\pslinewidth\psdoublesep\p@
\let\pst@setdoublesep\relax}
\def\tx@Shadow{Shadow }
\def\pst@closedshadow{%
  \addto@pscode{%
    gsave
    \psk@shadowsize \psk@shadowangle \tx@PtoC
    \tx@Shadow
    \pst@usecolor\psshadowcolor
    gsave fill grestore
    stroke
    grestore
    gsave
    \pst@usecolor\psfillcolor
    gsave fill grestore
    stroke
    grestore}}
%
\def\pst@openshadow{%
  \addto@pscode{%
    gsave
    \psk@shadowsize \psk@shadowangle \tx@PtoC
    \tx@Shadow
    \pst@usecolor\psshadowcolor
    \ifx\psk@fillstyle\relax\else
      gsave fill grestore
    \fi
    stroke}%
  \pst@repeatarrows%
  \addto@pscode{grestore}%
  \ifx\psk@fillstyle\relax\else
    \addto@pscode{%
      gsave
      \pst@usecolor\psfillcolor
      gsave fill grestore
      stroke
      grestore}%
  \fi}
%
\def\pst@addborder{%
  \addto@pscode{%
    gsave
    \psk@border 2 mul
    CLW add SLW
    \pst@usecolor\psbordercolor
    stroke
    grestore}}
%
\def\pst@stroke{%
  \ifx\pslinestyle\@none\else
    \addto@pscode{%
      gsave
      \pst@number\pslinewidth SLW
      \pst@usecolor\pslinecolor
      \tx@setStrokeTransparency % hv 2008-01-13
      \@nameuse{psls@\pslinestyle}
      grestore}%
  \fi}
%
\def\pst@fill#1{\addto@pscode{gsave #1 grestore}}%
%
\def\pst@doublestroke{%
    \addto@pscode{%
      gsave
      \psdoublesep SLW
      \pst@usecolor\psdoublecolor
      stroke
      grestore
}}
%
\def\pst@arrowtype{%
  \ifx\psk@arrowB\@empty 0 \else -2 \fi
  \ifx\psk@arrowA\@empty 0 \else -1 \fi
  add }
%
\def\pst@addarrowdef{%
  \addto@pscode{%
    /ArrowA {
      \ifx\psk@arrowA\@empty
        \pst@oplineto
      \else
        \pst@arrowdef{A}
        moveto
      \fi
    } def
    /ArrowB { \ifx\psk@arrowB\@empty \else \pst@arrowdef{B} \fi } def
}}
%
\def\pst@arrowdef#1{%
  \ifnum\pst@repeatarrowsflag>\z@
    /Arrow#1c [ 6 2 roll ] cvx def Arrow#1c
  \fi
  \tx@BeginArrow 
  \psk@arrowscale
  \@nameuse{psas@\@nameuse{psk@arrow#1}}
  \tx@EndArrow
}
%
\def\pst@repeatarrows{%
  \addto@pscode{%
    gsave
    \ifx\psk@arrowA\@empty\else ArrowAc ArrowA pop pop \fi
    \ifx\psk@arrowB\@empty\else ArrowBc ArrowB pop pop pop pop \fi
    grestore
}}
%
\def\pst@OpenShowPoints{%
  \addto@pscode{%
    gsave
    \psk@dotsize
    \@nameuse{psds@\psk@dotstyle}
    newpath
    Points aload length 2 div 2 sub cvi /N ED
    N 0 ge
      { \ifx\psk@arrowA\@empty Dot \else pop pop \fi 
        N { Dot } repeat 
	\ifx\psk@arrowB\@empty Dot \else pop pop \fi }
      { N 2 mul { pop } repeat } ifelse
    grestore
}}
%
\newif\ifPst@custom\Pst@customfalse
\define@boolkey[psset]{pstricks}[Pst@]{noCurrentPoint}[true]{}
\psset[pstricks]{noCurrentPoint=false}
%
%
\def\pscustom{\pst@object{pscustom}}
\long\def\pscustom@i#1{%
  \begin@SpecialObj%
  \solid@star%
  \let\pst@ifcustom\iftrue%
  \Pst@customtrue%
  \let\begin@ClosedObj\begin@CustomObj%
  \let\end@ClosedObj\endgroup%
  \def\begin@OpenObj{\begin@CustomObj\pst@addarrowdef}%
  \let\end@OpenObj\endgroup%
  \let\begin@AltOpenObj\begin@CustomObj%
  \def\begin@SpecialObj{%
    \begingroup%
    \pst@misplaced{special graphics object}%
    \def\addto@pscode####1{}%
    \let\end@SpecialObj\endgroup}%
  \def\@multips(##1)(##2)##3##4{\pst@misplaced\multips}%
  \def\psclip##1{\pst@misplaced\psclip}%
  \def\pst@repeatarrowsflag{\z@}%
  \let\pst@setrepeatarrowsflag\relax%
  \showpointsfalse%
  \def\pst@linetype{\pslinetype}%
  \def\psk@liftpen{\z@}%
%  \psset{liftpen=0}%
  \def\pst@cp{/currentpoint load stopped pop }%
  \def\pst@oplineto{/lineto load stopped { moveto } if }%
  \def\pst@optcp##1##2{\ifnum##1=\z@\def##2{/currentpoint load stopped { 0 0 } if }\fi}%
  \let\caddto@pscode\addto@pscode%
  \def\cuse@par##1{{\use@par##1}}%
  \the\pst@customdefs%
  \setbox\pst@hbox=\hbox{#1}%
  \psk@fillstyle
  \pst@stroke
  \end@SpecialObj
  \let\pst@ifcustom\iffalse
}
%
\let\pst@ifcustom\iffalse
%
\def\begin@CustomObj{%
  \begingroup%
  \use@par%
  \addto@pscode{
    \pst@number\pslinewidth SLW
    \pst@usecolor\pslinecolor
  }%
}
\def\pst@oplineto{moveto }
\def\pst@cp{}
\def\pst@optcp#1#2{}
\define@key[psset]{pstricks}{liftpen}[0]{%
  \ifPst@custom%
  \ifcase#1\relax%
    \def\psk@liftpen{\z@}%
    \def\pst@cp{/currentpoint load stopped pop }%
    \def\pst@oplineto{/lineto load stopped { moveto } if }%
  \or%
    \def\psk@liftpen{1}%
    \def\pst@cp{}%
    \def\pst@oplineto{/lineto load stopped { moveto } if }%
  \or%
    \def\psk@liftpen{2}%
    \def\pst@cp{}%
    \def\pst@oplineto{moveto }%
  \fi\fi%
}
\psset[pstricks]{liftpen=0}
\def\psk@liftpen{-1}
%
\define@key[psset]{pstricks}{linetype}[2]{%
  \pst@getint{#1}\pslinetype
  \ifnum\pst@cntg<-3
    \@pstrickserr{linetype must be greater than -3}\@ehpa
    \def\pslinetype{2}%
  \fi}
\psset[pstricks]{linetype=2}% otherwise there is a problem when using e.g.
%                     \psaxes[axesstyle=frame,linestyle=dashed]{->}(3,-2)
%
\def\caddto@pscode#1{%
    \@pstrickserr{Command can only be used in \string\pscustom}\@ehpa}
\let\cuse@par\caddto@pscode
%
\def\tx@MSave{%
     /msavematrx
         [ tx@Dict /msavematrx known % does msavematrix exists?
             { msavematrx aload pop } if
             CM % matrix currentmatrix
         ]
     def
%----------------- hv begin 2004-05-07 ------------- patch 15
    msavematrx
%----------------- hv end 2004-05-07 ------------- patch 15
}
\def\tx@MRestore{% a typo in pstricks with msavematrx
     tx@Dict /msavematrx known { length 0 gt } { false } ifelse
         { msavematrx aload pop setmatrix } if
}
%
\newtoks\pst@customdefs
\pst@customdefs{%
  \def\newpath{\addto@pscode{newpath}}%
  \def\reversepath{\addto@pscode{ reversepath }}%                      20131209  hv
  \def\moveto(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor moveto}}%
  \def\rmoveto(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor rmoveto}}%
  \def\closepath{\addto@pscode{closepath}}%
  \def\gsave{\begingroup\addto@pscode{gsave}}%
  \def\grestore{\endgroup\addto@pscode{grestore}}%
  \def\translate(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor translate}}%
  \def\rotate#1{\pst@@getangle{#1}\addto@pscode{\pst@angle rotate}}%
  \def\scale#1{\pst@getscale{#1}\pst@tempg\addto@pscode{\pst@tempg}}%
  \def\msave{\addto@pscode{\tx@MSave}}%
  \def\mrestore{\addto@pscode{\tx@MRestore}}%
  \def\swapaxes{\addto@pscode{-90 rotate -1 1 scale}}%
  \def\stroke{\def\pst@par{}\pst@object{stroke}}%
  \def\fill{\def\pst@par{}\pst@object{fill}}%
  \def\openshadow{\def\pst@par{}\pst@object{openshadow}}%
  \def\closedshadow{\def\pst@par{}\pst@object{closedshadow}}%
  \def\movepath(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor \tx@Shadow}}%
  \def\lineto{\pst@onecoor{lineto}}%
  \def\rlineto{\pst@onecoor{rlineto}}%
  \def\curveto{\pst@threecoor{curveto}}%
  \def\rcurveto{\pst@threecoor{rcurveto}}%
  \def\code#1{\addto@pscode{#1}}%
  \def\coor(#1){\pst@@getcoor{#1}\addto@pscode\pst@coor\@ifnextchar({\coor}{}}%
  \def\rcoor{\pst@getcoors{}{}}%
  \def\dim#1{\pssetlength\pst@dimg{#1}\addto@pscode{\pst@number\pst@dimg}}%
  \def\setcolor#1{%
    \@ifundefined{\string\color@#1}{}{\addto@pscode{\pst@usecolor{#1}}}}%  hv 1.14  2005-12-17
  \def\arrows#1{{\psset[pstricks]{arrows=#1}\pst@addarrowdef}}%
  \let\file\pst@rawfile%
} % END \pst@customdefs
%
\def\closedshadow@i{\cuse@par\pst@closedshadow}
\def\openshadow@i{\cuse@par\pst@openshadow}
\def\stroke@i{\cuse@par\pst@stroke}%
\def\fill@i{\cuse@par\psk@fillstyle}%
\def\pst@onecoor#1(#2){%
\pst@@getcoor{#2}%
\addto@pscode{\pst@coor #1}}
\def\pst@threecoor#1(#2)#3(#4)#5(#6){%
  \begingroup
    \pst@getcoor{#2}\pst@tempa
    \pst@getcoor{#4}\pst@tempb
% DG/SR modification begin - Aug.  4, 1999 - Patch 11
%\pst@getcoor{#6}\pst@tembc
    \pst@getcoor{#6}\pst@tempc
% DG/SR modification end
    \addto@pscode{\pst@tempa \pst@tempb \pst@tempc #1}%
  \endgroup}
%
\def\pst@rawfile#1{%
  \begingroup
  \def\do##1{\catcode`##1=12\relax}"
  \dospecials
  \catcode`\%=14
  \pst@@rawfile{#1}%
  \endgroup}
%
\def\pst@@rawfile#1{%
  \immediate\openin1 #1
  \ifeof1
    \@pstrickserr{File `#1' not found}\@ehpa
  \else
    \immediate\read1 to \pst@tempg
    \loop
      \ifeof1 \@pstfalse\else\@psttrue\fi
      \if@pst
      \addto@pscode\pst@tempg
      \immediate\read1 to \pst@tempg
    \repeat
  \fi
  \immediate\closein1\relax}
%
\def\tx@NArray{NArray }
\def\tx@Line{Line }
\def\tx@Arcto{Arcto }
\def\tx@CheckClosed{CheckClosed }
\def\tx@Polygon{Polygon }
\define@key[psset]{pstricks}{gangle}[0]{\pst@getangle{#1}\psk@gangle}
\define@boolkey[psset]{pstricks}[Pst@]{trueAngle}[true]{}
\psset[pstricks]{trueAngle=false,gangle=0}
%
\def\tx@Diamond{Diamond }
\def\psdiamond{\def\pst@par{}\pst@object{psdiamond}}
\def\psdiamond@i(#1){\@ifnextchar({\psdiamond@ii(#1)}{\psdiamond@ii(0,0)(#1)}}
\def\psdiamond@ii(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempa
  \pst@getcoor{#2}\pst@tempb
  \addto@pscode{%
    \psline@iii
    pop
    \psk@dimen
    \pst@tempb
    \psk@gangle
    \pst@tempa
    \tx@Diamond
  }%
  \def\pst@linetype{4}%
  \end@ClosedObj}
%
\def\tx@Triangle{Triangle }
\def\pstriangle{\def\pst@par{}\pst@object{pstriangle}}
\def\pstriangle@i(#1){\@ifnextchar({\pstriangle@ii(#1)}{\pstriangle@ii(0,0)(#1)}}
\def\pstriangle@ii(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempa%	the center of the baseline
  \pst@getcoor{#2}\pst@tempb%	the height of the triangle
  \addto@pscode{%
    \psline@iii
    pop			    %	no showpoints option
    \psk@dimen		    %	outer/inner/middle
    \pst@tempb
    \psk@gangle		    %	rotating angle
    \pst@tempa
    \tx@Triangle
  }%
  \def\pst@linetype{2}%
  \end@ClosedObj}
%
\def\tx@CCA{CCA }
\def\tx@CCA{CCA }
\def\tx@CC{CC }
\def\tx@IC{IC }
\def\tx@BOC{BOC }
\def\tx@NC{NC }
\def\tx@EOC{EOC }
\def\tx@BAC{BAC }
\def\tx@NAC{NAC }
\def\tx@EAC{EAC }
\def\tx@OpenCurve{OpenCurve }
\def\tx@AltCurve{AltCurve }
\def\tx@ClosedCurve{ClosedCurve }
%
\define@key[psset]{pstricks}{curvature}[1 0.1 0]{%
  \edef\pst@tempg{#1 }%
  \expandafter\psset@@curvature\pst@tempg * * * \@nil}
\def\psset@@curvature#1 #2 #3 #4\@nil{%
  \pst@checknum{#1}\pst@tempg
  \pst@checknum{#2}\pst@temph
  \pst@checknum{#3}\pst@tempi
  \edef\psk@curvature{\pst@tempg \pst@temph \pst@tempi}}
%
\psset[pstricks]{curvature=1 .1 0}
%
\def\pscurve{\pst@object{pscurve}}
\def\pscurve@i{%
  \pst@getarrows{%
    \begin@OpenObj
      \pst@getcoors[\pscurve@ii%
    }%
}
\def\pscurve@ii{%
  \addto@pscode{
    \ifPst@noCurrentPoint\else\pst@cp\fi		% current point
    \psk@curvature\space /c ED /b ED /a ED
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol \psls@symbol OpenSymbolCurve \else \tx@OpenCurve \fi
    \ifPst@variableLW \pst@flattenpath \fi
  }%
  \ifx\pslinestyle\psls@@symbol\def\pslinestyle{none}\fi%
  \end@OpenObj%
}
\def\psecurve{\pst@object{psecurve}}
\def\psecurve@i{\pst@getarrows{\begin@OpenObj\pst@getcoors[\psecurve@ii}}
\def\psecurve@ii{%
  \addto@pscode{
    \psk@curvature\space /c ED /b ED /a ED
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol \psls@symbol AltOpenSymbolCurve \else \tx@AltCurve \fi
  }%
  \ifx\pslinestyle\psls@@symbol\def\pslinestyle{none}\fi%
  \end@OpenObj}
%
\def\psccurve{\pst@object{psccurve}}
\def\psccurve@i{\begin@ClosedObj\pst@getcoors[\psccurve@ii}
\def\psccurve@ii{%
  \addto@pscode{%
    \psk@curvature\space /c ED /b ED /a ED
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol \psls@symbol ClosedSymbolCurve \else \tx@ClosedCurve \fi
  }%
  \def\pst@linetype{1}%
  \ifx\pslinestyle\psls@@symbol\def\pslinestyle{none}\fi%
  \end@ClosedObj}
%
\def\pscspline{\pst@object{pscspline}}%  Christoph Bersch
\def\pscspline@i{%
  \pst@getarrows{%
    \begin@OpenObj
    \pst@getcoors[\pscspline@ii
  }%
}
\def\tx@Spline{Spline }
\def\pscspline@ii{%
  \addto@pscode{
    \ifPst@noCurrentPoint\else\pst@cp\fi
    \tx@setlinejoin
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol 
      \psls@symbol OpenSymbolSpline
    \else
      \tx@Spline
    \fi
  }%      
  \end@OpenObj
}
%
\define@key[psset]{pstricks}{dotsize}[2pt 2]{%
  \pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil%
  \edef\psk@@dotsize{\pst@number\pst@dimg}%
  \let\psk@@@dotsize\pst@tempg%
  \edef\psk@dotsize{ /DS \psk@@dotsize \psk@@@dotsize CLW mul add 2 div def }}
\psset[pstricks]{dotsize=2pt 2}
%
\define@key[psset]{pstricks}{dotscale}[1]{%
  \pst@getscale{#1}\psk@dotscale
  \ifx\psk@dotscale\@empty
    \def\psk@xdotscale{1 }%
    \def\psk@ydotscale{1 }%
  \else
    \let\psk@xdotscale\pst@tempg
    \let\psk@ydotscale\pst@temph
  \fi}
%
\def\pst@Getangle#1#2{%
  \pst@getangle{#1}\pst@tempg
  \def\pst@temph{0. }%
  \ifx\pst@tempg\pst@temph\def#2{}\else\edef#2{\pst@tempg\space rotate }\fi}
%
\define@key[psset]{pstricks}{dotangle}[0]{%
  \pst@getangle{#1}\psk@@dotangle
  \ifdim\psk@@dotangle\p@=\z@
    \let\psk@dotangle\@empty
  \else
    \edef\psk@dotangle{\psk@@dotangle rotate }%
  \fi}
\psset[pstricks]{dotangle=0}
%
\def\pst@getdotsize{%
\pst@dimg=\psk@@@dotsize\pslinewidth
\advance\pst@dimg\psk@@dotsize\p@
\pst@dimh=\psk@ydotscale\pst@dimg
\pst@dimg=\psk@xdotscale\pst@dimg
\divide\pst@dimh 2
\divide\pst@dimg 2\relax}
%
\psset[pstricks]{dotscale=1}
%
\def\psdot{\pst@object{psdot}}
\def\psdot@i{\@ifnextchar({\psdot@ii}{\psdot@ii(\z@,\z@)}}
\def\psdot@ii(#1){%
  \begin@SpecialObj%
% hv modification 1.13 2005-11-28 
  \solid@star%
% hv modification end 
  \pst@@getcoor{#1}%
  \addto@pscode{
    \psk@dotsize
    \@nameuse{psds@\psk@dotstyle}
    \tx@setStrokeTransparency
    \pst@coor Dot}%
  \end@SpecialObj}
%
\def\psdots{\pst@object{psdots}}
\def\psdots@i{%
  \begin@SpecialObj%
  \pst@getcoors[\psdots@ii}
\def\psdots@ii{%
  \addto@pscode{ false \tx@NArray \psdots@iii }%
  \end@SpecialObj}
\def\psdots@iii{%
  \psk@dotsize
  \@nameuse{psds@\psk@dotstyle}
  \tx@setStrokeTransparency
  newpath
  n { transform floor .5 add exch floor .5 add exch itransform Dot  } repeat }
%
% DG: dead code (to suppress until \psset[pstricks]{dotstyle) ? - Aug. 4, 1997
\def\tx@SQ{SQ }
\def\tx@ST{ST }
\def\tx@SP{SP }
%
\def\pst@gdot#1{ /Dot { gsave T \psk@dotangle \psk@dotscale #1 grestore } def }
%
\@namedef{psds@*}{\pst@gdot{ 0 0 DS \tx@SD }}
\@namedef{psds@o}{%
  /r2 DS CLW sub def
  \pst@gdot{ 0 0 DS \tx@SD \pst@usecolor\psfillcolor SLW 0 0 r2 \tx@SD }}
\@namedef{psds@square*}{ /r1 DS .886 mul def \pst@gdot{r1 \tx@SQ }}
\@namedef{psds@square}{%
  /r1 DS .886 mul def /r2 r1 CLW sub def
  \pst@gdot{r1 \tx@SQ \pst@usecolor\psfillcolor r2 \tx@SQ}}
\@namedef{psds@triangle*}{%
  /y1 DS .778 mul neg def /x1 y1 1.732 mul neg def
  \pst@gdot{x1 y1 \tx@ST}}
\@namedef{psds@triangle}{%
  /y1 DS .778 mul neg def /x1 y1 1.732 mul neg def
  /y2 y1 CLW add def /x2 y2 1.732 mul neg def
  \pst@gdot{x1 y1 \tx@ST \pst@usecolor\psfillcolor x2 y2 \tx@ST}}
\@namedef{psds@pentagon*}{%
  /r1 DS 1.149 mul def
  \pst@gdot{r1 \tx@SP}}
\@namedef{psds@pentagon}{%
  DS .93 mul dup 1.236 mul /r1 ED CLW sub 1.236 mul /r2 ED
  \pst@gdot{r1 \tx@SP \pst@usecolor\psfillcolor r2 \tx@SP}}
\@namedef{psds@+}{%
  /DS DS 1.253 mul def
  \pst@gdot{DS 0 moveto DS neg 0 L stroke 0 DS moveto 0 DS neg L stroke}}
\@namedef{psds@|}{%
  \psk@tbarsize CLW mul add 2 div /DS ED
  \pst@gdot{0 DS moveto 0 DS neg L stroke}}
% DG: end dead code?
%
\define@key[psset]{pstricks}{dotstyle}[*]{%
  \@ifundefined{psds@#1}%
    {\@pstrickserr{Dot style `#1' not defined}\@eha}%
    {\edef\psk@dotstyle{#1}}}
\psset[pstricks]{dotstyle=*}
%
\def\tx@FontDot{FontDot }
\def\newpsfontdot#1[#2]#3#4{%
  \@namedef{psds@#1}{%
    /#3 \psk@@dotangle [#2] \tx@FontDot
% DG/SR modification begin - Dec. 12, 1999 - Patch 14
%/Dot { moveto #4 show } bind def }}
    /Dot { moveto gsave \psk@dotscale #4 show grestore } bind def 
}}
% DG/SR modification end
\def\newpsfontdotH#1[#2]#3#4#5{%	for filled objects
  \@namedef{psds@#1}{%
    /#3 \psk@@dotangle [#2] \tx@FontDot
    /Dot {
      moveto
%      \iftrue
% DG/SR modification begin - Dec. 23, 1999 - Patch 14
%gsave \pst@usecolor\psfillcolor #5 show grestore
%\fi
%#4 show
      gsave \psk@dotscale \pst@usecolor\psfillcolor #5 show grestore % fill first
%      \fi					
      gsave \psk@dotscale #4 show grestore	% show the unfilled one
% DG/SR modification end
    } bind def 
}}
%
\pstheader{pst-dots.pro}
\newpsfontdot{*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(b)}
\newpsfontdotH{o}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(c)}{(b)}
\newpsfontdotH{Bo}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(C)}{(b)}
\newpsfontdotH{triangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(t)}{(u)}
\newpsfontdotH{Btriangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(T)}{(u)}
\newpsfontdot{triangle*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(u)}
\newpsfontdotH{square}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(s)}{(r)}
\newpsfontdotH{Bsquare}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(S)}{(r)}
\newpsfontdot{square*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(r)}
\newpsfontdotH{pentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(p)}{(q)}
\newpsfontdotH{Bpentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(P)}{(q)}
\newpsfontdot{pentagon*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(q)}
% DG/SR modification begin - Mar. 18, 1997 and Dec. 16, 1999 - Patch 14
%\newpsfontdot{diamond*}[1.9 0.0 0.0 1.9 -0.4598 -0.70775]{Symbol}{<E0>}
%\newpsfontdot{diamond}[2.3 0.0 0.0 2.3 -0.8533 -0.5336]{Symbol}{<A8>}
% D.G. modification begin - Jan. 17, 2000
\newpsfontdotH{diamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(d)}{(l)}
\newpsfontdotH{Bdiamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(D)}{(l)}
\newpsfontdot{diamond*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(l)}
% DG/SR modification end
\newpsfontdot{oplus}[1.44928 0.0 0.0 1.44928 -0.562319 -0.478261]{Symbol}{<C5>}
\newpsfontdot{otimes}[1.44928 0.0 0.0 1.44928 -0.562319 -0.475362]{Symbol}{<C4>}
\newpsfontdot{x}[1.8 0.0 0.0 1.8 -0.495 -0.4788]{Symbol}{<B4>}
\newpsfontdot{+}[2.3 0.0 0.0 2.3 -0.6486 -0.5819]{Times-Roman}{<2B>}
\newpsfontdot{asterisk}[2.43309 0.0 0.0 2.43309 -0.609489 -1.14477]{Times-Roman}{<2A>}
\newpsfontdot{B+}[2.3 0.0 0.0 2.3 -0.6555 -0.5819]{Times-Bold}{<2B>}
\newpsfontdot{Basterisk}[2.29358 0.0 0.0 2.29358 -0.576835 -1.08486]{Times-Bold}{<2A>}
\newpsfontdot{|}[1.98413 0.0 0.0 1.38 -0.258929 -0.5]{Helvetica}{(|)}
% DG/SR modification begin - Oct. 27, 1997 - Patch 7
%[1.98413 0.0 0.0 1.98413 -0.258929 -0.712302]{Helvetica}{(|)}
% DG/SR modification end
\newpsfontdot{B|}[1.98413 0.0 0.0 1.38 -0.277778 -0.5]{Helvetica-Bold}{(|)}%
% DG/SR modification begin - Oct. 27, 1997 - Patch 7
%[1.98413 0.0 0.0 1.98413 -0.277778 -0.78302]{Helvetica-Bold}{(|)}

% DG/SR modification end
\iffalse
\newpsfontdot{*}[2.77778 0.0 0.0 2.77778 -0.638889 -0.813889]{Symbol}{<B7>}
\newpsfontdot{o}[3.33333 0.0 0.0 3.33333 -0.666667 -1.78167]{Symbol}{<B0>}
\newpsfontdot{Bo}[4.69484 0.0 0.0 4.69484 -0.78169 -2.97418]{Times-Bold}{<CA>}
\fi
% Etienne Riga
\newpsfontdot{Asterisk}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(k)}
\newpsfontdot{BoldAsterisk}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(K)}
\newpsfontdotH{SolidAsterisk}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(J)}{(b)}
%
\newpsfontdotH{Pentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(p)}{(q)}
\newpsfontdotH{BoldPentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(P)}{(q)}
\newpsfontdot{SolidPentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(q)}
\newpsfontdotH{Hexagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(h)}{(G)}
\newpsfontdotH{BoldHexagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(H)}{(G)}
\newpsfontdot{SolidHexagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(G)}
\newpsfontdotH{Octogon}[1 0 0 1 0 0]{PSTricksDotFont}{(f)}{(g)}
\newpsfontdotH{BoldOctogon}[1 0 0 1 0 0]{PSTricksDotFont}{(F)}{(g)}
\newpsfontdot{SolidOctogon}[1 0 0 1 0 0]{PSTricksDotFont}{(g)}
%
\newpsfontdot{Bullet}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(b)}
\newpsfontdotH{Circle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(c)}{(b)}
\newpsfontdotH{BoldCircle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(C)}{(b)}
%\newpsfontdot{SolidCircle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(u)}
\newpsfontdotH{Triangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(t)}{(u)}
\newpsfontdotH{BoldTriangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(T)}{(u)}
\newpsfontdot{SolidTriangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(u)}
\newpsfontdotH{Square}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(s)}{(r)}
\newpsfontdotH{BoldSquare}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(S)}{(r)}
\newpsfontdot{SolidSquare}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(r)}
\newpsfontdot{Add}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(a)}
\newpsfontdot{BoldAdd}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(A)}
\newpsfontdot{Mul}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(x)}
\newpsfontdot{BoldMul}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(X)}
\newpsfontdotH{Oplus}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(m)}{(b)}
\newpsfontdotH{BoldOplus}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(M)}{(b)}
\newpsfontdotH{SolidOplus}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(e)}{(b)}
\newpsfontdotH{Otimes}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(n)}{(b)}
\newpsfontdotH{BoldOtimes}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(N)}{(b)}
\newpsfontdotH{SolidOtimes}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(E)}{(b)}
\newpsfontdot{Bar}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(i)}
\newpsfontdot{BoldBar}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(I)}
\newpsfontdotH{Diamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(d)}{(l)}
\newpsfontdotH{BoldDiamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(D)}{(l)}
\newpsfontdot{SolidDiamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(l)}
%
\newdimen\pslinearc
\define@key[psset]{pstricks}{linearc}[0pt]{\pssetlength\pslinearc{#1}}
\psset[pstricks]{linearc=0pt}
%
\def\psline{\pst@object{psline}}
\def\psline@i{%
  \pst@getarrows{%
    \begin@OpenObj
    \pst@getcoors[\psline@ii%
  }%
}
\def\psline@ii{%
  \ifx\pslinestyle\psls@@symbol\addto@pscode{ \psls@symbol SymbolLine }%
  \else%
    \addto@pscode{
      \ifPst@noCurrentPoint\else\pst@cp\fi 	  % current point?
      \psline@iii % arc and lineto type
      \tx@Line	  % .pro function
    }%
  \fi%
  \end@OpenObj%
}
\def\psline@iii{%
  \ifdim\pslinearc>\z@
    /r \pst@number\pslinearc def
    /Lineto { \tx@Arcto } def
  \else
    /Lineto /lineto load def
  \fi
  \tx@setlinejoin 			% hv 2007-10-13
  \ifshowpoints true \else false \fi
}
%
\def\pst@isnum#1{\pst@isnum@i\zap@space#1 \@empty\@nil}%
\def\pst@isnum@i#1\@nil{%
  \if!\ifnum9<1#1!\else_\fi%
      \expandafter\@firstoftwo%
  \else%
      \expandafter\@secondoftwo%
  \fi}
%
\def\psset@@symbol#1#2#3#4\@nil{%
  \ifx\relax#4\relax\def\psk@symbol{(#1)}%
  \else%
    \pst@isnum{#1#2#3}{%
      \pst@cnta='#1#2#3\relax%
      \ifnum\pst@cnta>'377\relax%
        \@pstrickserr{Number too large!}\@ehpb%
      \else%
        \def\psk@symbol{(\@backslashchar#1#2#3)}%
      \fi%
}{\@pstrickserr{Not a number!}\@ehpb}%
  \fi}
%
\define@key[psset]{pstricks}{symbol}[a]{\expandafter\psset@@symbol#1!!\@nil}
\psset[pstricks]{symbol=a}
%
\newdimen\pst@symbolStep
\define@key[psset]{pstricks}{symbolStep}[20pt]{\pst@expandafter\pst@@symbolStep#1\@nil}
\def\pst@@symbolStep#1#2\@nil{\if-#1\pssetlength\pst@symbolStep{-#2pt}\else\pssetlength\pst@symbolStep{#1#2}\fi}
\psset[pstricks]{symbolStep=20pt}

\newdimen\pst@symbolWidth
\newdimen\pst@symbolLinewidth
\define@key[psset]{pstricks}{symbolWidth}[10pt]{\pssetlength\pst@symbolWidth{#1}}
\define@key[psset]{pstricks}{symbolLinewidth}[0.5pt]{\pssetlength\pst@symbolLinewidth{#1}}
\psset[pstricks]{symbolWidth=10pt,symbolLinewidth=0.5pt}

\define@key[psset]{pstricks}{symbolFont}[Dingbats]{\def\psk@symbolFont{/#1 }}
\psset[pstricks]{symbolFont=Dingbats}
\define@boolkey[psset]{pstricks}[Pst@]{rotateSymbol}[true]{}
\psset[pstricks]{rotateSymbol=false}
\define@key[psset]{pstricks}{startAngle}[0]{\pst@getangle{#1}\psk@startAngle}
\define@key[psset]{pstricks}{tickAngle}[0]{\pst@getangle{#1}\psk@tickAngle}
\psset[pstricks]{startAngle=0,tickAngle=0}
\define@boolkey[psset]{pstricks}[Pst@]{curveticks}[true]{}
\psset[pstricks]{curveticks=false}

%
\def\psls@symbol{
  /Symbol \psk@symbol def
  /SymbolWidth \pst@number\pst@symbolWidth def
  /SymbolLinewidth \pst@number\pst@symbolLinewidth def
  /SymStep \pst@number\pst@symbolStep def
  \psk@symbolFont findfont %0. [1.0 0.0 0.0 1.0 0.0 0.0]
  \pst@number\pst@symbolWidth scalefont %dup 
  setfont 
  /rotateSymbol \ifPst@rotateSymbol true \else false \fi def
  /tickAngle \psk@tickAngle\space def
  /startAngle \psk@startAngle\space def
  /CorrAngle \ifx\psk@rot\@empty 0 \else \psk@rot \fi def
  /curveticks \ifPst@curveticks true \else false \fi def
  \pst@number\pslinewidth SLW
}
\def\psls@@symbol{symbol}
%
\def\psPline{\def\pst@par{}\pst@object{psPline}}% perpendicular to another line B-C
\def\psPline@i{%
  \pst@getarrows{%
    \begin@OpenObj
    \pst@getcoors[\psPline@ii}%   \pst@coors on stack
}
\def\psPline@ii{%
  \addto@pscode{ % [ pC pB pA  is on stack
    /yA ED /xA ED
    /yB ED /xB ED
    yB sub exch xB sub div /mBC ED		% the slope
    /mA 1 mBC neg div def			% orthogonal
    /xS yA yB sub mBC xB mul add mA xA mul sub mBC mA sub div def
    /yS mBC xS xB sub mul yB add def
    xS yS xA yA 
    \ifPst@noCurrentPoint\else\pst@cp\fi 	% current point
    \psline@iii % arc and lineto type
    \tx@Line	% .pro function
  }%
  \end@OpenObj%
  \ignorespaces%
}
%
\def\qline(#1)(#2){%
  \def\pst@par{}%
  \begin@SpecialObj
  \def\pst@linetype{0}%
  \pst@getcoor{#1}\pst@tempa
  \pst@@getcoor{#2}%
  \addto@pscode{%
    \pst@tempa moveto \pst@coor L
    \@nameuse{psls@\pslinestyle}%
  }%
  \end@SpecialObj}
%
\def\pspolygon{\pst@object{pspolygon}}
\def\pspolygon@i{%
  \begin@ClosedObj%
  \def\pst@cp{}%
  \pst@getcoors[\pspolygon@ii%
}
\def\pspolygon@ii{%
  \ifx\pslinestyle\psls@@symbol\addto@pscode{ \psls@symbol SymbolPolygon }%
  \else                        \addto@pscode{\psline@iii \tx@Polygon}%
  \fi%
  \def\pst@linetype{1}%
  \end@ClosedObj}
%
\define@key[psset]{pstricks}{framearc}[0]{\pst@checknum{#1}\psk@framearc}
\psset[pstricks]{framearc=0}
%
\define@key[psset]{pstricks}{cornersize}[relative]{\pst@expandafter\psset@@cornersize{#1}\@nil}
\def\psset@@cornersize#1#2\@nil{%
  \if #1a\relax
    \def\psk@cornersize{\pst@number\pslinearc false }%
  \else\def\psk@cornersize{\psk@framearc true }%
  \fi}
\psset[pstricks]{cornersize=relative}
%
\def\tx@Rect{Rect }
\def\tx@OvalFrame{OvalFrame }
\def\tx@Frame{Frame }
%
\define@key[psset]{pstricks}{dimen}[outer]{\pst@expandafter\psset@@dimen{#1}\@nil}
\def\psset@@dimen#1#2\@nil{%
  \if #1o\relax%	outer
    \def\psk@dimen{.5 }%
  \else
    \if #1m\relax%	middle
      \def\psk@dimen{0 }%
    \else
      \if #1i\relax%	inner
        \def\psk@dimen{-.5 }%
  \fi\fi\fi}
\psset[pstricks]{dimen=outer}
%
\def\psframe{\pst@object{psframe}}
\def\psframe@i(#1){%
  \@ifnextchar({\psframe@ii(#1)}{\psframe@ii(0,0)(#1)}}
\def\psframe@ii(#1)(#2){%
  \begin@ClosedObj
    \pst@getcoor{#1}\pst@tempa
    \pst@@getcoor{#2}%
    \addto@pscode{ \psk@cornersize \pst@tempa \pst@coor \psk@dimen \tx@Frame }%
    \def\pst@linetype{2}%
    \showpointsfalse
  \end@ClosedObj
}

\iffalse
\def\psSquare{\pst@object{psSquare}}
\def\psSquare@i(#1)(#2){%
  \begin@ClosedObj
    \pst@getcoor{#1}\pst@tempa
    \pst@getcoor{#2}\pst@tempb
    \addto@pscode{ \psk@cornersize 
      \pst@tempa /yA ED /xA ED 
      \pst@tempb /yB ED /xB ED
      xA yA moveto xB yB L
      xA xB sub yA yB sub atan /Angle ED
      xA yA xB yB Pyth2 dup xA add exch yA add 
      \psk@dimen 
      \tx@Frame 
%      grestore
    }%
    \def\pst@linetype{2}%
    \showpointsfalse
  \end@ClosedObj
}
\fi
%
\def\psTextFrame{\pst@object{psTextFrame}}
\def\psTextFrame@i(#1)(#2)#3{%
  \addbefore@par{ref=c}%	to prevent an empty value
  \leavevmode%
  \pst@killglue
  \begingroup
  \use@par
  \ifx\psk@yref\relax \def\psk@yref{0}\fi% no Baseline possible
  \SpecialCoor
  \pst@getcoor{#1}\pst@tempA
  \pst@getcoor{#2}\pst@tempB
  \if@star\psframe*(#1)(#2)\else\psframe(#1)(#2)\fi
  \rput(! \pst@tempA \pst@tempB % x1 y1 x2 y2
    exch 4 -1 roll 		% y1 y2 x2 x1
    dup /x1 ED			% y1 y2 x2 x1
    sub /dx ED			% y1 y2 
    exch dup /y1 ED 		% y2 y1
    sub /dy ED	
    x1 dx \psk@xref\space mul add \pst@number\psxunit div 
    y1 dy \psk@yref\space mul add \pst@number\psyunit div ){#3}
  \endgroup
  \ignorespaces}
%
\def\tx@BezierNArray{ BezierNArray }
\def\tx@OpenBezier{ OpenBezier }
\def\tx@ClosedBezier{ ClosedBezier }
\def\tx@BezierShowPoints{ BezierShowPoints }
\def\tx@BezierCurve{ BezierCurve }
\def\pst@BezierType{2 }	% the default
%
\def\psbezier{\pst@object{psbezier}}
\def\psbezier@i{%
  \pst@getarrows{%
    \begin@OpenObj
      \pst@getcoors[\psbezier@ii%
  }%
}
\def\psbezier@ii{%
  \addto@pscode{
    \ifPst@noCurrentPoint\else\pst@cp\fi
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol \psls@symbol OpenSymbolBezier 
    \else 
      \tx@OpenBezier 
      \ifshowpoints \tx@BezierShowPoints \fi
    \fi
  }%
  \def\pst@linetype{1}%
  \ifx\pslinestyle\psls@@symbol\def\pslinestyle{none}\fi%
  \end@OpenObj}
%
\def\pscbezier{\def\pst@par{}\pst@object{pscbezier}}
\def\pscbezier@i{%
  \begin@ClosedObj
  \pst@getcoors[\pscbezier@ii}
%
\def\pscbezier@ii{%
  \addto@pscode{%
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol \psls@symbol ClosedSymbolBezier 
    \else 
      \tx@ClosedBezier
      \ifshowpoints \tx@BezierShowPoints \fi
    \fi}%
%  \chardef\pst@linetype=1
  \def\pst@linetype{1}%
  \ifx\pslinestyle\psls@@symbol\def\pslinestyle{none}\fi%
  \end@ClosedObj}
%
\iffalse
\define@key[psset]{pstricks}{epsilon}[0.005]{\pst@checknum{#1}\psk@epsilon}
\psset[pstricks]{epsilon=0.005}		% 200 steps for one curve
%
\def\psBezier#1{%		% allowed order is 1 ... 9
  \ifnum#1>0 \ifnum#1<10 \def\pst@BezierType{#1 }\fi\fi%
  \def\pst@par{}\pst@object{psBezier}}
\def\psBezier@i{%
  \pst@getarrows{%
    \begin@OpenObj
    \pst@getcoors[\psBezier@ii%
}}
\def\psBezier@ii{%
  \addto@pscode{%
    \psk@epsilon	    	% step for Bezier T=0,0+epsilon,0+i*epsilon,...,1
    \pst@BezierType 		% type of the Bezier curve 2,3,4,... 
    \tx@BezierCurve
    \ifshowpoints \tx@BezierShowPoints \fi
  }%
  \end@OpenObj}
\fi
%
\define@key[psset]{pstricks}{pType}[0]{\pst@cntg=#1\relax\edef\psk@pType{\the\pst@cntg}}
\psset[pstricks]{pType=0}
\def\tx@Parab{Parab }%	 given by 1 point and the min/max
\def\tx@Parabo{Parab1 }% given by 2 points for y-a=(x-b)^2
%
\def\psparabola{\pst@object{psparabola}}%  2009-05-19 (hv)
\def\psparabola@i{\pst@getarrows\psparabola@ii}
\def\psparabola@ii#1(#2)#3(#4){%  #2 P #4 SP
  \begin@OpenObj
  \pst@getcoor{#2}\pst@tempa
  \pst@@getcoor{#4}%
  \addto@pscode{\pst@tempa \pst@coor 
    \ifcase\psk@pType
      \tx@Parab \or
      \tx@Parabo
    \fi}%
  \end@OpenObj}
\let\parabola\psparabola% compatibility  (hv)
%
%
\define@key[psset]{pstricks}{gridwidth}[0.8pt]{\pst@getlength{#1}\psk@gridwidth}
\psset[pstricks]{gridwidth=.8pt}
\define@key[psset]{pstricks}{griddots}[0]{%
  \pst@cntg=#1\relax
  \edef\psk@griddots{\the\pst@cntg}}
\psset[pstricks]{griddots=0}
\define@key[psset]{pstricks}{gridcolor}[black]{\pst@getcolor{#1}\psgridcolor}
\psset[pstricks]{gridcolor=black}
\define@key[psset]{pstricks}{subgridwidth}[0.4pt]{\pst@getlength{#1}\psk@subgridwidth}
\psset[pstricks]{subgridwidth=0.4pt}
\define@key[psset]{pstricks}{subgridcolor}[gray]{\pst@getcolor{#1}\pssubgridcolor}
\psset[pstricks]{subgridcolor=gray}
\define@key[psset]{pstricks}{subgriddots}[0]{%
  \pst@cntg=#1\relax\edef\psk@subgriddots{\the\pst@cntg}}
\psset[pstricks]{subgriddots=0}
\define@key[psset]{pstricks}{subgriddiv}[5]{%
  \pst@cntg=#1\relax\edef\psk@subgriddiv{\the\pst@cntg}}
\psset[pstricks]{subgriddiv=5}
%
\define@key[psset]{pstricks}{gridfont}[Helvetica]{\def\psk@gridfont{/#1 }}%   hv 2007-11-13
\psset[pstricks]{gridfont=Helvetica}
%
\define@key[psset]{pstricks}{gridlabels}[10pt]{\pst@getlength{#1}\psk@gridlabels}
\psset[pstricks]{gridlabels=10pt}
\define@key[psset]{pstricks}{gridlabelcolor}[black]{\pst@getcolor{#1}\psgridlabelcolor}
\psset[pstricks]{gridlabelcolor=black}

\def\tx@Grid{Grid }

\def\psgrid{\pst@object{psgrid}}
\def\psgrid@i{\@ifnextchar({\psgrid@ii}{\expandafter\psgrid@iv\pic@coor}}
\def\psgrid@ii(#1){\@ifnextchar({\psgrid@iii(#1)}{\psgrid@iv(0,0)(0,0)(#1)}}
\def\psgrid@iii(#1)(#2){\@ifnextchar({\psgrid@iv(#1)(#2)}{\psgrid@iv(#1)(#1)(#2)}}
\def\psgrid@iv(#1)(#2)(#3){%
  \begin@SpecialObj%
    \pst@getcoor{#1}\pst@tempA%  hv 1.11
    \pst@getcoor{#2}\pst@tempB%  hv 1.11
    \pst@@getcoor{#3}%
    \ifnum\psk@subgriddiv>1\relax
      \addto@pscode{
        gsave
        \tx@setStrokeTransparency
        \psk@subgridwidth SLW 
        \pst@usecolor\pssubgridcolor
        \pst@tempB \pst@coor \pst@tempA                 % hv 1.11
%        \pst@number\psxunit \pst@number\psyunit        % hv 1.11
        \pst@number\psxunit abs \pst@number\psyunit abs % hv 1.11
        \psk@subgriddiv\space \psk@subgriddots\space
        {} 0 
        \psk@gridfont findfont 0 scalefont setfont      % hv 1.16
	\tx@Grid 
	grestore
      }%
    \fi%
    \addto@pscode{
      gsave
      \tx@setStrokeTransparency
      \psk@gridwidth SLW 
      \pst@usecolor\psgridcolor
      \pst@tempB \pst@coor \pst@tempA                 % hv 1.11
      \pst@number\psxunit abs \pst@number\psyunit abs % hv 1.11
%      \pst@number\psxunit \pst@number\psyunit        % hv 1.11
      1 \psk@griddots\space { \pst@usecolor\psgridlabelcolor }
      \psk@gridlabels 
      \psk@gridfont findfont \psk@gridlabels scalefont setfont  % hv 1.16
       \tx@Grid 
      grestore
    }%
  \end@SpecialObj}
%
\newif\ifpsmathbox
\psmathboxtrue
\def\pst@mathflag{\z@}
\newtoks\everypsbox
\let\pst@thisbox\relax
%
\long\def\pst@makenotverbbox#1#2{%
  \edef\pst@mathflag{%
  \ifpsmathbox\ifmmode\ifinner 1\else 2\fi\else\z@\fi\else\z@\fi}%
  \setbox\pst@hbox=\hbox{%
    \ifcase\pst@mathflag\or$\m@th\textstyle\or$\m@th\displaystyle\fi%
    {\pst@thisbox\the\everypsbox#2}%
    \ifnum\pst@mathflag>\z@$\fi%                                     $
  }%
  #1}
%
\def\pst@makeverbbox#1{%
  \def\pst@afterbox{#1}%
  \edef\pst@mathflag{\ifpsmathbox\ifmmode\ifinner1\else2\fi\else\z@\fi\else\z@\fi}%
  \afterassignment\pst@beginbox%
  \setbox\pst@hbox\hbox%
}
\def\pst@beginbox{%
  \ifcase\pst@mathflag\or$\m@th\or$\m@th\displaystyle\fi%
  \bgroup\aftergroup\pst@endbox%
  \pst@thisbox%
  \the\everypsbox%
}
\def\pst@endbox{%
  \ifnum\pst@mathflag>\z@\relax$\fi%                      $
  \egroup%
  \pst@afterbox%
}
\def\pst@makebox{\pst@@makebox}
\def\psverbboxtrue{\def\pst@@makebox{\pst@makeverbbox}}
\def\psverbboxfalse{\def\pst@@makebox{\pst@makenotverbbox}}
\psverbboxfalse
\def\pst@longbox{%
  \def\pst@makebox{%
    \gdef\pst@makebox{\pst@@makebox}%
    \pst@makelongbox%
  }%
}
\def\pst@makelongbox#1{%
  \def\pst@afterbox{#1}%
  \edef\pst@mathflag{%
    \ifpsmathbox\ifmmode\ifinner 1\else 2\fi\else \z@\fi\else \z@\fi%
  }%
  \setbox\pst@hbox\hbox\bgroup
  \aftergroup\pst@afterbox
  \ifcase\pst@mathflag\or$\m@th\or$\m@th\displaystyle\fi
  \begingroup
  \pst@thisbox
  \the\everypsbox%
}
\def\pst@endlongbox{%
  \endgroup
  \ifnum\pst@mathflag>\z@$\fi		%$
  \egroup%
}
\def\pslongbox#1#2{%
  \@namedef{#1}{\pst@longbox#2}%
  \@namedef{end#1}{\pst@endlongbox}}
%
\newdimen\psframesep
\define@key[psset]{pstricks}{framesep}[3pt]{\pssetlength\psframesep{#1}}
\psset[pstricks]{framesep=3pt}
%
\define@boolkey[psset]{pstricks}[ps]{boxsep}[true]{}
\psset[pstricks]{boxsep}
%
\def\pst@useboxpar{%
  \use@par%
  \if@star%
    \let\pslinecolor\psfillcolor%
    \solid@star%
    \let\solid@star\relax
  \fi%
  \ifpsdoubleline \pst@setdoublesep \fi}
%
\def\psframebox{\def\pst@par{}\pst@object{psframebox}}
\def\psframebox@i{\pst@makebox\psframebox@ii}
\def\psframebox@ii{%
  \begingroup
  \pst@useboxpar
  \pst@dima=\pslinewidth
  \advance\pst@dima by \psframesep
  \pst@dimc=\wd\pst@hbox\advance\pst@dimc by \pst@dima
  \pst@dimb=\dp\pst@hbox\advance\pst@dimb by \pst@dima
  \pst@dimd=\ht\pst@hbox\advance\pst@dimd by \pst@dima
  \setbox\pst@hbox=\hbox{%
    \ifpsboxsep\kern\pst@dima\fi
    \begin@ClosedObj
    \addto@pscode{%
      \psk@cornersize % arcradius boolean
      \pst@number\pst@dima neg
      \pst@number\pst@dimb neg
      \pst@number\pst@dimc
      \pst@number\pst@dimd
      .5
      \tx@Frame%
    }%
    \def\pst@linetype{2}%
    \showpointsfalse
    \end@ClosedObj
    \box\pst@hbox
    \ifpsboxsep\kern\pst@dima\fi%
  }%
  \ifpsboxsep\dp\pst@hbox=\pst@dimb\ht\pst@hbox=\pst@dimd\fi
  \leavevmode\box\pst@hbox
  \endgroup}
%
\def\psdblframebox{\def\pst@par{}\pst@object{psdblframebox}}
\def\psdblframebox@i{\addto@par{doubleline=true}\psframebox@i}
%
\define@key[psset]{pstricks}{clipcommand}[clip]{\def\pst@clipcommand{#1 }}
\psset[pstricks]{clipcommand=clip}% alternative is eoclip
%
\def\psclip{\@ifnextchar[\psclip@i{\psclip@i[]}}%
\def\psclip@i[#1]#2{%
  \leavevmode%
  \begingroup%
    \ifx\relax#1\relax\else\psset{#1}\fi%
    \begin@psclip%
      \begingroup%
        \def\use@pscode{%
          \pstVerb{
            \pst@dict
            /mtrxc CM def
            CP CP T
            \tx@STV
            \psk@origin
            \psk@swapaxes
            newpath
            \pst@code
            \pst@clipcommand
            newpath
            mtrxc setmatrix
            moveto
            0 setgray
            end
	  }%
          \gdef\pst@code{}}%
  \def\@multips(##1)(##2)##3##4{\pst@misplaced\multips}%
  \def\nc@object##1##2##3##4{\pst@misplaced{node connection}}%
  \hbox to\z@{#2}%
  \endgroup%
  \def\endpsclip{%
    \end@psclip%
    \endgroup}%
  \ignorespaces}
%
\def\endpsclip{\pst@misplaced\endpsclip}
\let\begin@psclip\relax
\def\end@psclip{\pstVerb{currentpoint initclip moveto}}
%
\def\AltClipMode{%
  \def\end@psclip{\pstVerb{\pst@grestore}}%
  \def\begin@psclip{\pstVerb{gsave}}}
  \def\clipbox{\@ifnextchar[{\clipbox@}{\clipbox@[\z@]}}
% DG modification begin - Apr. 3, 1997
% From paulus@immd5.informatik.uni-erlangen.de (Dietrich Paulus)
%\def\clipbox@[#1]{\pst@makebox\clipbox@@{#1}}
\def\clipbox@[#1]{\pst@makebox{\clipbox@@{#1}}}
% DG modification end
\def\clipbox@@#1{%
  \pssetlength\pst@dimg{#1}%
  \leavevmode\hbox{%
  \begin@psclip%
  \pst@Verb{
    CM \tx@STV CP T newpath
    /a \pst@number\pst@dimg def
    /w \pst@number{\wd\pst@hbox}a add def
    /d \pst@number{\dp\pst@hbox}a add neg def
    /h \pst@number{\ht\pst@hbox}a add def
    a neg d moveto
    a neg h L
    w h L
    w d L
    closepath
    \pst@clipcommand
    newpath
    0 0 moveto
    setmatrix}%
  \unhbox\pst@hbox%
  \end@psclip}}
%
\def\psshadowbox{\def\pst@par{}\pst@object{psshadowbox}}
\def\psshadowbox@i{\pst@makebox\psshadowbox@ii}
\def\psshadowbox@ii{%
\begingroup
\pst@useboxpar
\psshadowtrue
\psboxseptrue
\def\psk@shadowangle{-45 }%
\setbox\pst@hbox=\hbox{\psframebox@ii}%
\pst@dimh=\psk@shadowsize\p@
\pst@dimh=.7071\pst@dimh
\pst@dimg=\dp\pst@hbox
\advance\pst@dimg\pst@dimh
\dp\pst@hbox=\pst@dimg
\pst@dimg=\wd\pst@hbox
\advance\pst@dimg\pst@dimh
\wd\pst@hbox=\pst@dimg
\leavevmode
\box\pst@hbox
\endgroup}
%
\def\pscirclebox{\pst@object{pscirclebox}}
\def\pscirclebox@i{\pst@makebox\pscirclebox@ii}
\def\pscirclebox@ii{%
\begingroup%
\pst@useboxpar%
\setbox\pst@hbox=\hbox{%
\pst@nodehook%
\pscirclebox@iii%
\box\pst@hbox}%
\ifpsboxsep\pscirclebox@sep\fi%
\leavevmode%
\box\pst@hbox%
\endgroup}
%
\def\pscirclebox@iii{%
  \if@star%
    \pslinewidth\z@%
    \pstverb{\pst@dict \tx@STP \pst@usecolor\psfillcolor
             newpath \pscirclebox@iv \tx@SD end}%
  \else%
    \begin@ClosedObj%
    \def\pst@linetype{4}\showpointsfalse%
    \addto@pscode{ \pscirclebox@iv\space CLW 2 div add 0 360 arc closepath}%
    \end@ClosedObj%
  \fi}
%
\def\pscirclebox@iv{
  \pst@number{\wd\pst@hbox} 2 div
  \pst@number{\ht\pst@hbox} \pst@number{\dp\pst@hbox} add 2 div
  2 copy \pst@number{\dp\pst@hbox} sub 4 2 roll
  \tx@Pyth \pst@number\psframesep add }
%
\def\pscirclebox@sep{%
  \pst@dimn=\ht\pst@hbox%			% the height of the box
  \advance\pst@dimn by \dp\pst@hbox%		% the depth  of the box added to \pst@dimn
  \divide\pst@dimn by 2%			% \pst@dimn/2
  \pst@dimm=0.5\wd\pst@hbox%			% the half of the width
  \pst@Pyth\pst@dimm\pst@dimn\pst@dimo%		% the diameter
  \advance\pst@dimo by \pslinewidth%
  \advance\pst@dimo by \psframesep%
  \advance\pst@dimn by -\pst@dimo%
  \setbox\pst@hbox=\hbox to 2\pst@dimo{\hss\vbox{\kern-\pst@dimn\box\pst@hbox}\hss}%
  \advance\pst@dimn by -\dp\pst@hbox%
  \dp\pst@hbox=-\pst@dimn}
%  
\let\pst@nodehook\relax
%
\def\psCirclebox{\def\pst@par{}\pst@object{psCirclebox}}
\def\psCirclebox@i{\pst@makebox\psCirclebox@ii}
\def\psCirclebox@ii{%
  \begingroup
  \pst@useboxpar
  \pst@dima=\ht\pst@hbox
  \advance\pst@dima\dp\pst@hbox
  \divide\pst@dima\tw@
  \pssetlength\pst@dimb\psk@radius
  \setbox\pst@hbox=\hbox{%
    \pst@nodehook
    \pscircle(.5\wd\pst@hbox,\pst@dima){\pst@dimb}%
    \box\pst@hbox}%
  \ifpsboxsep \psCirclebox@sep \fi
  \leavevmode
  \box\pst@hbox
  \endgroup}
%
\def\psCirclebox@sep{%
  \pst@dimc=\pst@dimb
  \advance\pst@dimb-\pst@dima
  \advance\pst@dima\pst@dimc
  \setbox\pst@hbox=\hbox to\tw@\pst@dimc{%
    \hss\vrule width \z@ depth \pst@dimb height \pst@dima
    \box\pst@hbox\hss}}
%
\def\psovalbox{\def\pst@par{}\pst@object{psovalbox}}
\def\psovalbox@i{\pst@makebox{\psovalbox@ii}}
\def\psovalbox@ii{%
  \begingroup
  \pst@useboxpar
  \psovalbox@iii
  \ifpsboxsep\psovalbox@sep\fi
  \leavevmode
  \box\pst@hbox
  \endgroup}
%
\def\psovalbox@iii{%
  \psovalbox@iv
  \setbox\pst@hbox=\hbox{%
    \begin@ClosedObj
    \addto@pscode{%
      0 360
      \pst@number\pst@dimc CLW 2 div sub
      \pst@number\pst@dimd CLW 2 div sub
      \pst@number\pst@dima
      \pst@number\pst@dimb
      \tx@Ellipse
      closepath }%
    \def\pst@linetype{2}%
    \end@ClosedObj
    \unhbox\pst@hbox}}
%
\def\psovalbox@iv{%
  \pst@dimc=\pslinewidth\advance\pst@dimc\psframesep
  \pst@dimd=\ht\pst@hbox\advance\pst@dimd\dp\pst@hbox
  \pst@dima=.5\wd\pst@hbox
  \pst@dimb=.5\pst@dimd\advance\pst@dimb-\dp\pst@hbox
  \pst@dimd=.707\pst@dimd
  \advance\pst@dimd\pst@dimc
  \advance\pst@dimc.707\wd\pst@hbox}
%
\def\psovalbox@sep{%
  \setbox\pst@hbox\hbox to 2\pst@dimc{\hss\unhbox\pst@hbox\hss}%
  \pst@dimg=\pst@dimd
  \advance\pst@dimg-\pst@dimb
  \dp\pst@hbox=\pst@dimg
  \advance\pst@dimd\pst@dimb
  \ht\pst@hbox=\pst@dimd}
%
\def\psdiabox{\def\pst@par{}\pst@object{psdiabox}}
\def\psdiabox@i{\pst@makebox{\psdiabox@ii}}
\def\psdiabox@ii{%
\begingroup
\pst@useboxpar
\psdiabox@iii
\ifpsboxsep\psdiabox@sep\fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\psdiabox@iv{%
\pst@dimg=.707\pslinewidth
\advance\pst@dimg.707\psframesep
\pst@dima=\wd\pst@hbox
\divide\pst@dima 2
\pst@dimc=\pst@dima
\advance\pst@dimc\pst@dimg
\pst@dimd=\ht\pst@hbox
\advance\pst@dimd\dp\pst@hbox
\divide\pst@dimd 2
\pst@dimb=\pst@dimd
\advance\pst@dimb-\dp\pst@hbox
\advance\pst@dimd\pst@dimg}
\def\psdiabox@iii{%
\psdiabox@iv
\setbox\pst@hbox=\hbox{%
\begin@ClosedObj
\addto@pscode{%
\psline@iii
pop
.5
\pst@number\pst@dimc 2 mul \pst@number\pst@dimd 2 mul
0
\pst@number\pst@dima \pst@number\pst@dimb
\tx@Diamond}%
\def\pst@linetype{4}%
\end@ClosedObj
\box\pst@hbox}}
\def\psdiabox@sep{%
\setbox\pst@hbox\hbox to 4\pst@dimc{\hss\unhbox\pst@hbox\hss}%
\multiply\pst@dimd 2
\advance\pst@dimd\pst@dimb
\ht\pst@hbox\pst@dimd
\advance\pst@dimd-2\pst@dimb
\dp\pst@hbox\pst@dimd}
%
\define@key[psset]{pstricks}{trimode}[U]{\pst@expandafter\psset@@trimode{#1}\@empty\@empty\@nil}
\def\psset@@trimode#1#2#3\@nil{%
  \let\pst@tempg#1\relax
  \ifx\pst@tempg*
    \let\psk@@trimode\@empty
    \let\pst@tempg#2\relax
  \else
    \let\psk@@trimode\relax
  \fi
  \edef\psk@trimode{%
    \ifx R\pst@tempg 1 % Right
    \else
      \ifx D\pst@tempg 2 % Down
      \else
        \ifx L\pst@tempg 3 % Left
        \else 
          \ifx l\pst@tempg 4 % |_
          \else
            \ifx r\pst@tempg 5 % _|
            \else 0 \fi     % Up
          \fi
        \fi
      \fi
    \fi}%
}
\psset[pstricks]{trimode=U}
%
\def\pstribox{\pst@object{pstribox}}
\def\pstribox@i{\pst@makebox{\pstribox@ii}}
\def\pstribox@ii{%
  \begingroup
  \pst@useboxpar
  \pstribox@iii
  \ifpsboxsep\pstribox@sep\fi
  \leavevmode
  \box\pst@hbox
  \endgroup}
%
\def\pstribox@iii{%
  \pstribox@iv
  \setbox\pst@hbox=\hbox{%
    \begin@ClosedObj
    \addto@pscode{
      \psline@iii
      pop
      0.5
      \pst@number\pst@dimc % Width
      \pst@number\pst@dimd % Height
      \ifcase\psk@trimode  
             \or  %% 0
        exch \or  %% 1
             \or  %% 2
        exch \or  %% 3
             \or  %% 4
             \or  %% 5
      \fi
      \psk@trimode -90 mul
      \pst@number\pst@dima % x coor for text
      \pst@number\pst@dimb % y coor for text
      \tx@Triangle}%
    \def\pst@linetype{2}%
    \end@ClosedObj
    \box\pst@hbox}%
}
%
\def\pstribox@iv{%
  \pst@dimh=\pslinewidth
  \advance\pst@dimh\psframesep
  \pst@dimg=\ht\pst@hbox
  \advance\pst@dimg-\dp\pst@hbox         % totalheight
  \divide\pst@dimg 2                     % 0.5 totalheight
  \edef\pst@tempa{\number\pst@dimg sp}%  % For use by nodes.
  \ifodd\psk@trimode                     % 
    \pst@dimb\pst@dimg
  \else
    \pst@dima=\wd\pst@hbox
    \divide\pst@dima 2
  \fi
  \ifcase\psk@trimode
    \pst@dimb=-\dp\pst@hbox
    \advance\pst@dimb-\pst@dimh
  \or\pst@dima=-\pst@dimh
  \or\pst@dimb=\ht\pst@hbox
     \advance\pst@dimb\pst@dimh
  \or\pst@dima=\wd\pst@hbox
     \advance\pst@dima\pst@dimh
  \fi
  \pst@dimd=\dp\pst@hbox
  \advance\pst@dimd\ht\pst@hbox
  \ifx\psk@@trimode\relax% no star for trimode=
    \pst@dimc=\wd\pst@hbox
    \advance\pst@dimc\ifodd\psk@trimode 1.447\else 1.789\fi\pst@dimh
    \multiply\pst@dimc 2
    \advance\pst@dimd\ifodd\psk@trimode 1.789\else 1.447\fi\pst@dimh
    \multiply\pst@dimd 2
  \else% trimode=R*,L*,U*,D*
    \ifodd\psk@trimode
      \advance\pst@dimd 1.1547\wd\pst@hbox
      \advance\pst@dimd 3.4641\pst@dimh
      \pst@dimc=.866\pst@dimd
    \else
      \advance\pst@dimd .866\wd\pst@hbox %.866=(sqrt(3)/2)
      \advance\pst@dimd 3\pst@dimh 
      \pst@dimc=1.1547\pst@dimd % 1.1547=(2/sqrt(3))
    \fi
  \fi}
%
\def\pstribox@sep{%
\ifodd\psk@trimode
\advance\pst@dimb.5\pst@dimd
\ht\pst@hbox=\pst@dimb
\advance\pst@dimd-\pst@dimb
\dp\pst@hbox=\pst@dimd
\else
\setbox\pst@hbox\hbox to \pst@dimc{\hss\unhbox\pst@hbox\hss}%
\global\pst@dimg=.5\pst@dimc
\fi
\ifcase\psk@trimode
\dp\pst@hbox-\pst@dimb
\advance\pst@dimd\pst@dimb
\ht\pst@hbox\pst@dimd
\or
\pst@dimg=.5\wd\pst@hbox
\global\advance\pst@dimg-\pst@dima
\setbox\pst@hbox\hbox to \pst@dimc{\kern-\pst@dima\box\pst@hbox\hss}%
\or
\ht\pst@hbox\pst@dimb
\advance\pst@dimd-\pst@dimb
\dp\pst@hbox\pst@dimd
\or
\pst@dimg=\pst@dimc
\advance\pst@dimg-\pst@dima
\global\advance\pst@dimg.5\wd\pst@hbox
\setbox\pst@hbox\hbox to \pst@dimc{%
\hss\box\pst@hbox\kern\psframesep\kern\pslinewidth}%
\fi}
%
\define@key[psset]{pstricks}{arcsepA}[0]{\pst@getlength{#1}\psk@arcsepA}
\define@key[psset]{pstricks}{arcsepB}[0]{\pst@getlength{#1}\psk@arcsepB}
\define@key[psset]{pstricks}{arcsep}[0]{%
  \pst@getlength{#1}\psk@arcsepA\let\psk@arcsepB\psk@arcsepA}
\psset[pstricks]{arcsep=0}
\def\tx@ArcArrow{ArcArrow }
%
\def\psarc{\pst@object{psarc}}
\def\psarc@i{\@ifnextchar({\psarc@iii}{\psarc@ii}}
\def\psarc@ii#1{\addto@par{arrows=#1}\@ifnextchar(\psarc@iii{\psarc@iii(0,0)}}
\def\psarc@iii(#1)#2#3#4{%
  \begin@OpenObj%
    \pst@getangle{#3}\pst@tempa%
    \pst@getangle{#4}\pst@tempb%
    \ifx\pst@tempa\pst@tempb\else%
      \pst@@getcoor{#1}%
      \pssetlength\pst@dima{#2}%
      \addto@pscode{\psarc@iv \psarc@v
        \ifPst@variableLW \pst@flattenpath \fi
      }%
      \gdef\psarc@type{0}%
      \showpointsfalse%
    \fi%
  \end@OpenObj%
}
\def\psarc@iv{%
  \pst@coor /y ED /x ED
  /r \ifPst@SpecialLength \pst@SpecialLength \else \pst@number\pst@dima \fi def
  /c 57.2957 r \tx@Div def
  /angleA
    \pst@tempa
    \psk@arcsepA c mul 2 div
    \ifcase\psarc@type add \or sub \fi
  def
  /angleB
    \pst@tempb
    \psk@arcsepB c mul 2 div
    \ifcase\psarc@type sub \or add \fi
  def
  \ifshowpoints\psarc@showpoints\fi
  \ifx\psk@arrowA\@empty
    \ifnum\psk@liftpen=2
      r angleA \tx@PtoC
      y add exch x add exch moveto
    \fi
  \fi}
% hv ---- 1.10 2005-05-05 ----------------------> hv begin
\def\psarc@v{%
  /angleAtoB angleB angleA gt { true }{ false } ifelse def
  x y r
  angleA
  \ifx\psk@arrowA\@empty\else
    { ArrowA CP }
    r 0 gt \pslbrace
    { \ifcase\psarc@type add \or sub \fi } \psrbrace\pslbrace
    { \ifcase\psarc@type sub \or add \fi } \psrbrace ifelse
%    { \ifcase\psarc@type add \or sub \fi }
    \tx@ArcArrow
%    dup AngleA gt AngleAtoB exor { neg } fi
  \fi
  angleB
  \ifx\psk@arrowB\@empty\else
    { ArrowB }
    r 0 gt \pslbrace
      { \ifcase\psarc@type sub \or add \fi } \psrbrace\pslbrace
      { \ifcase\psarc@type add \or sub \fi } \psrbrace ifelse
%      { \ifcase\psarc@type sub \or add \fi }
    \tx@ArcArrow
    dup angleA gt angleAtoB xor { pop angleA } if
  \fi
\ifcase\psarc@type arc \or arcn \fi}
% hv ----- 1.10 2005-05-05 ------------------------> end
%
\def\psarc@type{0}
\def\psarc@showpoints{%
  gsave
  newpath
  x y moveto
  x y r \pst@tempa \pst@tempb
  \ifcase\psarc@type arc \or arcn \fi
  closepath
  CLW 2 div SLW
  [ \psk@dash\space ] 0 setdash stroke
  grestore }
\def\psarcn{\def\pst@par{}\pst@object{psarcn}}
\def\psarcn@i{\def\psarc@type{1}\psarc@i}
%
\def\psarcAB{\pst@object{psarcAB}}%		hv 2008-11-26
\def\psarcAB@i{%
  \addbefore@par{psscale=1}% be sure, that it is defined
  \pst@getarrows{%
    \begin@OpenObj%
      \pst@getcoors{}\psarcAB@ii%
    }%
}
\def\psarcAB@ii{%
  \addto@pscode{
  /y ED /x ED /yA ED /xA ED /yB ED /xB ED 
  /r xB yB x y Pyth2 \psk@psscale\space mul def
  /c 57.2957 r \tx@Div def
  /angleA
    yA y sub xA x sub atan
    \psk@arcsepA c mul 2 div
    \ifcase\psarc@type add \else sub \fi
  def
  /angleB
    yB y sub xB x sub atan
    \psk@arcsepB c mul 2 div
    \ifcase\psarc@type sub \else add \fi 
  def
  \ifx\psk@arrowA\@empty
    \ifnum\psk@liftpen=2
      r angleA \tx@PtoC
      y add exch x add exch moveto
    \fi
  \fi
  \psarc@v }%
  \gdef\psarc@type{0}%
  \showpointsfalse%
  \end@OpenObj%
}
\def\psarcnAB{\def\pst@par{}\pst@object{psarcnAB}}
\def\psarcnAB@i{\def\psarc@type{1}\psarcAB@i}
%
%------------------ tvz/DG/hv (2004-05-10) begin -------------------%%
% from Denis Giroux: http://www.tug.org/pipermail/pstricks/2001/000507.html
%
% I - Definition of \psellipticwedge, a generalization of \pswedge for wedges
%     of ellipses (from the code of \pswedge and \psellipse)
%
\def\psellipticwedge{\pst@object{psellipticwedge}}
\def\psellipticwedge@i(#1){%
  \@ifnextchar({\psellipticwedge@ii(#1)}{\psellipticwedge@ii(0,0)(#1)}}
\def\psellipticwedge@ii(#1)(#2)#3#4{%
  \begin@ClosedObj
    \pst@getangle{#3}\pst@tempa
    \pst@getangle{#4}\pst@tempb
    \pst@getcoor{#1}\pst@tempc
    \pst@@getcoor{#2}%
    \def\pst@linetype{1}%
    \addto@pscode{%
      \pst@coor /ry ED /rx ED
      \ifx\psk@rot\@empty \else \psk@rot\space rotate \fi
      \pst@tempa 
      \ifPst@correctAngle
       cvi 90 mod 0 eq { \pst@tempa } 
         { rx abs ry abs sub cvi 0 eq { \pst@tempa }{ rx ry
           \tx@UserCoor exch \pst@tempa tan mul exch atan 
            \pst@tempa 180 div 0.5 add floor 
            180 mul sub } ifelse } ifelse
      \fi
      \pst@tempb
      \ifPst@correctAngle
       cvi 90 mod 0 eq { \pst@tempb } 
         { rx abs ry abs sub cvi 0 eq { \pst@tempb }{ rx ry
           \tx@UserCoor exch \pst@tempb tan mul exch atan 
            \pst@tempb 180 div 0.5 add floor 
            180 mul sub } ifelse } ifelse
      \fi
      rx ry
      \pst@tempc moveto
      \ifdim\psk@dimen\p@=\z@\else
        \psk@dimen CLW mul dup 3 1 roll
        sub 3 1 roll sub exch
      \fi
      \pst@tempc
      \tx@Ellipse
      closepath
    }%
  \showpointsfalse
  \end@ClosedObj%
}
%
% Code mainly from "pstricks.tex'' 0.94 beta (TvZ)
%
\def\psellipticarcn{\pst@object{psellipticarcn}}
\def\psellipticarcn@i{\let\if@psarcn\iftrue\psellipticarc@ii}
%
\def\psellipticarc{\pst@object{psellipticarc}}
\def\psellipticarc@i{\let\if@psarcn\iffalse\psellipticarc@ii}
\define@boolkey[psset]{pstricks}[Pst@]{correctAngle}[true]{}
\psset{correctAngle}

\let\if@psarcn\iffalse

\def\psellipticarc@ii{\pst@getarrows\psellipticarc@iii}
\def\psellipticarc@iii(#1){%
  \@ifnextchar({\psellipticarc@iv(#1)}{\psellipticarc@iv(0,0)(#1)}}
\def\psellipticarc@iv(#1)(#2)#3#4{%
%  \addbefore@par{correctAngle=false}
  \begin@OpenObj%
  \pst@getcoor{#1}\pst@tempa    %	origin
  \pst@getcoor{#2}\pst@tempb	%	a b
  \pst@getangle{#3}\pst@tempc	%	start angle
  \pst@getangle{#4}\pst@tempd	% 	end angle
  \addto@pscode{ 
    \psellipticarc@definearg \psellipticarc@draw
    \ifPst@variableLW \pst@flattenpath \fi 
  }%
  \ifshowpoints
    \addto@pscode{
      gsave
      xOrig yOrig T % set origin to ellipse origin
      \ifx\psk@rot\@empty \else \psk@rot\space rotate \fi
      rx ry scale   % now we draw a circle :-)
      1 \pst@tempc  % start angle
      \ifPst@correctAngle
       cvi 90 mod 0 eq { \pst@tempc } 
         { rx abs ry abs sub cvi 0 eq { \pst@tempc }{ rx ry
           \tx@UserCoor exch \pst@tempc tan mul exch atan 
            \pst@tempc 180 div 0.5 add floor 
            180 mul sub } ifelse } ifelse
      \fi
      PtoC moveto 
      0 0 lineto 
      1 \pst@tempd % end angle
      \ifPst@correctAngle
       cvi 90 mod 0 eq { \pst@tempd } 
         { rx ry \tx@UserCoor exch \pst@tempd tan mul exch atan 
            \pst@tempd 180 div .5 add floor 180 mul sub } ifelse 
      \fi
      PtoC lineto
   %  \ifcase\psarc@type arc \or arcn \fi
      CLW 2 div SLW 
      [ 1 1 \tx@UserCoor ] 0 setdash 
      stroke
      grestore 
    }
  \showpointsfalse%
  \fi
  \end@OpenObj%
}
\def\psellipticarc@definearg{%
%  \ifx\psk@rot\@empty \else \psk@rot\space rotate \fi
  \pst@tempa /yOrig ED /xOrig ED  % Origin
  \pst@tempb                      % radii. Now adjust:
  \ifdim\psk@dimen\p@=\z@\else
    \psk@dimen CLW mul dup 3 1 roll
    sub 3 1 roll sub exch
  \fi
  /ry ED /rx ED		% a b
  /angleA
    /d { \if@psarcn sub \else add \fi } def
%    \pst@tempc 
% the angle in the parameter equation is not proportional to the real angle!
% phi=atan(b*tan(angle)/a)+floor(angle/180+0.5)*180
   \pst@tempc 
   \ifPst@correctAngle 
     cvi 90 mod 0 eq { \pst@tempc } 
       { rx ry \tx@UserCoor exch \pst@tempc tan mul exch atan 
          \pst@tempc 180 div .5 add floor 180 mul sub } ifelse 
    \fi
    \psk@arcsepA 2 div
    ArcAdjust
  def
  /angleB
    /d { \if@psarcn add \else sub \fi } def
%    \pst@tempd 
  \pst@tempd 
  \ifPst@correctAngle
     cvi 90 mod 0 eq { \pst@tempd } 
       { rx ry \tx@UserCoor exch \pst@tempd tan mul exch atan 
          \pst@tempd 180 div .5 add floor 180 mul sub } ifelse 
  \fi
  \psk@arcsepB 2 div ArcAdjust  def
%  \ifshowpoints\psellipticarc@showpoints\fi
  \ifx\psk@arrowA\@empty
    \ifnum\psk@liftpen=2
      angleA cos rx mul xOrig add
      angleA sin ry mul yOrig add
      moveto
    \fi%
  \fi%
}
\def\psellipticarc@draw{%
  0 0 1
  angleA
  \ifx\psk@arrowA\@empty\else
    { ArrowA CP }
    { \if@psarcn sub \else add \fi }
    EllipticArcArrow
  \fi
  angleB
  \ifx\psk@arrowB\@empty\else
    { ArrowB }
    { \if@psarcn add \else sub \fi }
    EllipticArcArrow
  \fi
  /mtrx CM def
  xOrig yOrig T
  \ifx\psk@rot\@empty \else \psk@rot\space rotate \fi
  rx ry scale
  \pst@ifcustom\else
    0 0 moveto 
    exch dup dup               % end start start start
    cos exch sin moveto        % end start
    exch                       % start end 
  \fi
%%  \if@star 0 0 moveto \fi	% for filling
  \if@psarcn arcn \else arc \fi
%%  \if@star 0 0 moveto \fi
  mtrx setmatrix%
}
\def\psellipticarc@showpoints{%
  gsave
  /mtrx CM def
  xOrig yOrig T
  rx ry scale
  0 0 moveto
  0 0 1 
  \pst@tempc % start angle
  \ifPst@correctAngle
     cvi 90 mod 0 eq { \pst@tempc } 
       { rx abs ry abs sub cvi 0 eq { \pst@tempc }{ rx ry
         \tx@UserCoor exch \pst@tempc tan mul exch atan 
          \pst@tempc 180 div 0.5 add floor 
          180 mul sub } ifelse } ifelse
    \fi
  \pst@tempd % end angle
   \ifPst@correctAngle
     cvi 90 mod 0 eq { \pst@tempd } 
       { rx abs ry abs sub cvi 0 eq { \pst@tempd } { rx ry 
         \tx@UserCoor exch \pst@tempd tan mul exch atan 
          \pst@tempd 180 div 0.5 add floor 
          180 mul sub } ifelse } ifelse
    \fi
  \ifcase\psarc@type arc \or arcn \fi
  closepath
  mtrx setmatrix
  CLW 2 div SLW
  [ \psk@dash\space ] 0 setdash 
  stroke
  grestore %
}
\def\pscircle{\def\pst@par{}\pst@object{pscircle}}
\def\pscircle@i{\@ifnextchar({\pscircle@do}{\pscircle@do(0,0)}}
\def\pscircle@do(#1)#2{%
  \if@star{\use@par\qdisk(#1){#2}}%   	qdisk does not allow
  \else%				to use opacity option
    \begin@ClosedObj
    \pst@@getcoor{#1}%
    \pssetlength\pst@dimc{#2}%
    \def\pst@linetype{4}%
    \addto@pscode{
      \pst@coor 2 copy moveto
      \ifPst@SpecialLength \pst@SpecialLength \else \pst@number\pst@dimc \fi      
      \psk@dimen CLW mul sub
      dup 0 rmoveto
      0 360 arc
      \ifPst@variableLW \pst@flattenpath \fi
      closepath
    }%
    \showpointsfalse
    \end@ClosedObj
  \fi
  \ignorespaces}
%
\def\pscircleOA{\def\pst@par{}\pst@object{pscircleOA}}%	hv 2008-04-14
\def\pscircleOA@i(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempA
  \pst@@getcoor{#2}%
  \def\pst@linetype{4}%
  \addto@pscode{
    \pst@tempA			% x0 y0
    2 copy			% xO yO xO yO 
    \pst@coor			% xO yO xO yO xA yA 
    Pyth2			% xO yO radius
    \psk@dimen CLW mul sub
    \if@star \tx@SD \else
      0 360 arc
      closepath 
    \fi }%
  \showpointsfalse
  \end@ClosedObj
  \ignorespaces}
%
\def\qdisk(#1)#2{%
  \def\pst@par{}%
  \begin@SpecialObj
  \pst@@getcoor{#1}%
  \pssetlength\pst@dimg{#2}%
  \addto@pscode{ 
    \pst@coor 
    \ifPst@SpecialLength \pst@SpecialLength \else \pst@number\pst@dimg \fi
%    \pst@number\pst@dimg 
    \tx@SD }%
  \end@SpecialObj}
%
\define@key[psset]{pstricks}{radius}[0.25cm]{\pst@@getlength{#1}\psk@radius}
\psset[pstricks]{radius=.25cm}
%
\def\psCircle{\pst@object{psCircle}}% same as \pscircle, but uses \psk@radius
\def\psCircle@i{\@ifnextchar({\psCircle@ii}{\psCircle@ii(0,0)}}
\def\psCircle@ii(#1){\pscircle@do(#1){\psk@radius}}
%
\def\psRing{\def\pst@par{}\pst@object{psRing}}%% hv 20130405
\def\psRing@i{\@ifnextchar({\psRing@ii}{\psRing@ii(0,0)}}
\def\psRing@ii(#1){%
  \pst@@getcoor{#1}%
  \@ifnextchar[{\psRing@iii}{\psRing@iii[0,360]}}
\def\psRing@iii[#1,#2]#3#4{%   origin, inner radius, outer radius
  \begin@ClosedObj
  \pssetlength\pst@dimc{#3}%
  \pssetlength\pst@dimd{#4}%
  \pst@getangle{#1}\pst@tempa
  \pst@getangle{#2}\pst@tempb
  \def\pst@linetype{4}%
  \addto@pscode{
    \pst@coor translate 
    \pst@number\pst@dimc \psk@dimen CLW mul sub /InnerRadius ED
    \pst@number\pst@dimd \psk@dimen CLW mul sub /OuterRadius ED
    InnerRadius 0 moveto newpath
    0 0 InnerRadius \pst@tempa\space \pst@tempb\space arc 
    OuterRadius \pst@tempb\space PtoC 
    \pst@tempb\space \pst@tempa\space sub abs 360 eq { moveto }{ lineto } ifelse % whole circle or not??
    0 0 OuterRadius \pst@tempb\space \pst@tempa\space arcn 
    closepath
  }%
  \showpointsfalse
  \end@ClosedObj
  \ignorespaces}
%
\def\pswedge{\def\pst@par{}\pst@object{pswedge}}
\def\pswedge@i{\@ifnextchar({\pswedge@ii}{\pswedge@ii(0,0)}}
\def\pswedge@ii(#1)#2#3#4{%
  \begin@ClosedObj%
  \pssetlength\pst@dimc{#2}%
  \pst@getangle{#3}\pst@tempa%
  \pst@getangle{#4}\pst@tempb%
  \pst@@getcoor{#1}%
  \def\pst@linetype{1}%
  \addto@pscode{
    \ifx\psk@rot\@empty 0 \else \psk@rot \fi rotate
    \pst@coor
    2 copy
    moveto
    \ifPst@SpecialLength \pst@SpecialLength \else \pst@number\pst@dimc \fi
%    \pst@number\pst@dimc 
    \psk@dimen CLW mul sub % Adjusted radius
    \pst@tempa \pst@tempb
    arc
    closepath}%
  \showpointsfalse%
  \end@ClosedObj%
}
\def\tx@ellipse#1{ \ifx\psk@rot\@empty 0 \else \psk@rot \fi #1  Ellipse }
\def\tx@Ellipse{ \ifx\psk@rot\@empty 0 \else \psk@rot \fi Ellipse }
%
\def\psellipse{\def\pst@par{}\pst@object{psellipse}}
\def\psellipse@i(#1){\@ifnextchar({\psellipse@ii(#1)}{\psellipse@ii(0,0)(#1)}}
\def\psellipse@ii(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempa
  \pst@@getcoor{#2}%
  \addto@pscode{
    0 360
    \pst@coor 
    \ifdim\psk@dimen\p@=\z@\else
      \psk@dimen CLW mul
      dup 4 -1 roll sub neg 3 1 roll sub
    \fi
    \pst@tempa 
    \tx@ellipse{true}
    \ifPst@variableLW \pst@flattenpath \fi
    closepath
  }%
  \def\pst@linetype{2}%
  \end@ClosedObj%
}
\def\psellipseAB{\def\pst@par{}\pst@object{psellipseAB}}
\def\psellipseAB@i(#1)(#2)#3{%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempa
  \pst@getcoor{#2}\pst@tempb
  \addto@pscode{
    0 360
    #3 \pst@number\psxunit mul
    \pst@tempa /yA ED /xA ED
    \pst@tempb /yB ED /xB ED
    xA xB sub dup mul
    yA yB sub dup mul add sqrt 2 div
    \ifdim\psk@dimen\p@=\z@\else
      \psk@dimen CLW mul
      dup 4 -1 roll sub neg 3 1 roll sub
    \fi
    xA xB add 2 div yA yB add 2 div
    translate 0 0
    xB xA sub yA yB sub atan 
    Ellipse  % on stack is rotate coordinates
    \ifPst@variableLW \pst@flattenpath \fi
    closepath
  }%
  \def\pst@linetype{2}%
  \end@ClosedObj
}
\def\multips{\@ifnextchar({\def\pst@par{}\multips@ii}{\multips@i}}
\def\multips@i#1{\def\pst@par{rot=#1}\multips@ii}
\def\multips@ii(#1){\@ifnextchar({\multips@iii(#1)}{\multips@iii(\z@,\z@)(#1)}}
\long\def\multips@iii(#1)(#2)#3#4{%
  \begingroup
%----------------- hv 1.10 ------------------
  \pst@killglue
%----------------- hv 1.10 ------------------
  \use@par
  \pst@getcoor{#1}\pst@tempa
  \pst@@getcoor{#2}%
  \pst@cnta=#3\relax
  \init@pscode
  \addto@pscode{%
    \pst@tempa T \the\pst@cnta\space \pslbrace
    gsave \ifx\psk@rot\@empty\else\psk@rot rotate \fi}%
  \hbox to\z@{%
    \def\init@pscode{%
      \addto@pscode{%
        gsave
        \pst@number\pslinewidth SLW
        \pst@usecolor\pslinecolor}}%
    \def\use@pscode{\addto@pscode{grestore}}%
    \def\psclip##1{\pst@misplaced\psclip}%
    \def\nc@object##1##2##3##4{\pst@misplaced{node connection}}%
    #4%
  }%
  \addto@pscode{grestore \pst@coor T \psrbrace repeat}%
  \leavevmode
  \use@pscode
  \endgroup
  \ignorespaces}
\def\psscalebox#1{\pst@makebox{\ps@scalebox{#1}}}
\def\ps@scalebox#1{%
  \begingroup%
  \pst@getscale{#1}\pst@tempa%
  \let\pst@tempc\pst@tempg%
  \let\pst@tempd\pst@temph%
  \ps@@scalebox%
  \endgroup}
\def\ps@@scalebox{%
  \leavevmode%
  \hbox{%
    \ifdim\pst@tempd\p@<\z@%
      \pst@dimg=\pst@tempd\ht\pst@hbox%
      \pst@dimh=\pst@tempd\dp\pst@hbox%
      \dp\pst@hbox=-\pst@dimg%
      \ht\pst@hbox=-\pst@dimh%
    \else%
      \ht\pst@hbox=\pst@tempd\ht\pst@hbox%
      \dp\pst@hbox=\pst@tempd\dp\pst@hbox%
    \fi%
    \pst@dima=\pst@tempc\wd\pst@hbox%
    \ifdim\pst@dima<\z@\kern-\pst@dima\fi%
    \pst@Verb{CP CP translate \pst@tempa \tx@NET}%
    \hbox to \z@{\box\pst@hbox\hss}%
    \pst@Verb{
      CP CP translate
      1 \pst@tempc div 1 \pst@tempd div scale
      \tx@NET}%
    \ifdim\pst@dima>\z@\kern\pst@dima\fi%
  }%
}
\pslongbox{Scalebox}{\psscalebox}
%
\def\psscaleboxto(#1,#2){\pst@makebox{\ps@scaleboxto(#1,#2)}}
\def\ps@scaleboxto(#1,#2){%
  \begingroup
  \pssetlength\pst@dima{#1}%
  \pssetlength\pst@dimb{#2}%
  \ifdim\pst@dima=\z@\else
    \pst@divide{\pst@dima}{\wd\pst@hbox}\pst@tempc
    \edef\pst@tempc{\pst@tempc\space}%
  \fi
  \ifdim\pst@dimb=\z@
    \ifdim\pst@dima=\z@
      \@pstrickserr{%
        \string\psscaleboxto\space dimensions cannot both be zero}\@ehpa
      \def\pst@tempa{}%
      \def\pst@tempc{1 }%
      \def\pst@tempd{1 }% 
    \else
      \let\pst@tempd\pst@tempc
    \fi
  \else
    \pst@dimc=\ht\pst@hbox
    \advance\pst@dimc\dp\pst@hbox
    \pst@divide{\pst@dimb}{\pst@dimc}\pst@tempd
    \edef\pst@tempd{\pst@tempd\space}%
    \ifdim\pst@dima=\z@ \let\pst@tempc\pst@tempd \fi
  \fi
  \edef\pst@tempa{\pst@tempc \pst@tempd scale }%
  \ps@@scalebox
  \endgroup}
\pslongbox{Scaleboxto}{\psscaleboxto}
%
\def\tx@Rot{Rot }
\def\psrotateleft{\pst@makebox{\ps@rotateleft\pst@hbox}}
\def\ps@rotateleft#1{%
\leavevmode\hbox{\hskip\ht#1\hskip\dp#1\vbox{\vskip\wd#1%
\pst@Verb{90 \tx@Rot}
\vbox to \z@{\vss\hbox to \z@{\box#1\hss}\vskip\z@}%
\pst@Verb{-90 \tx@Rot}}}}
\def\psrotateright{\pst@makebox{\ps@rotateright\pst@hbox}}
\def\ps@rotateright#1{%
% ----------- hv begin 2004-05-07 ----------- patch 15
%    \hbox{%
  \leavevmode\hbox{%
% ----------- hv end 2004-05-07 ----------- patch 15
  \hskip\ht#1\hskip\dp#1\vbox{\vskip\wd#1%
  \pst@Verb{-90 \tx@Rot}
  \vbox to \z@{\hbox to \z@{\hss\box#1}\vss}%
  \pst@Verb{90 \tx@Rot}}}}
\def\psrotatedown{\pst@makebox{\ps@rotatedown\pst@hbox}}
\def\ps@rotatedown#1{%
\hbox{\hskip\wd#1\vbox{\vskip\ht#1\vskip\dp#1%
\pst@Verb{180 \tx@Rot}%
\vbox to \z@{\hbox to \z@{\box#1\hss}\vss}%
\pst@Verb{-180 \tx@Rot}}}}
\pslongbox{Rotateleft}{\psrotateleft}
\pslongbox{Rotateright}{\psrotateright}
\pslongbox{Rotatedown}{\psrotatedown}
% ----------- hv begin 2004-09-23 ----------- 1.11
% compatibility stuff 
\let\rotateleft\psrotateleft
\let\rotateright\psrotateright
\let\rotatedown\psrotatedown
% ----------- hv end 2005-09-23 ----------- 1.11
\def\pst@starbox{%
\setbox\pst@hbox\hbox{\psframebox*[boxsep=false]{\unhbox\pst@hbox}}}
\def\pst@@makesmall#1{%
\setbox#1=\hbox to\z@{\hss\vbox to \z@{\vss\box#1\vss}\hss}}
\def\pst@@@makesmall#1{%
\pst@dimh=\psk@xref\wd#1%
\ifx\psk@yref\relax
\pst@dimg=\dp#1%
\else
\pst@dimg=\psk@yref\ht#1%
\advance\pst@dimg\psk@yref\dp#1%
\fi
\setbox#1=\hbox to\z@{%
\kern-\pst@dimh\vbox to\z@{\vss\box#1\kern-\pst@dimg}\hss}}
%
\define@key[psset]{pstricks}{ref}[c]{\pst@expandafter\psset@@ref{#1}\@empty,,\@nil}
\def\psset@@ref#1#2,#3,#4\@nil{%
  \def\psk@xref{.5}%
  \def\psk@yref{.5}%
  \let\pst@makesmall\pst@@@makesmall
  \ifx\@empty#3\@empty
    \@nameuse{getref@#1}%
    \@nameuse{getref@#2}%
  \else
    \pst@checknum{#1#2}\psk@xref
    \pst@checknum{#3}\psk@yref
  \fi}
%
\def\getref@c{\let\pst@makesmall\pst@@makesmall}
\def\getref@t{\def\psk@yref{1}}
\def\getref@b{\def\psk@yref{0}}
\def\getref@B{\let\psk@yref\relax}
\def\getref@l{\def\psk@xref{0}}
\def\getref@r{\def\psk@xref{1}}
\psset[pstricks]{ref=c}
%
\def\pst@rotlist{ mark RAngle /ps@a ED cleartomark ps@a neg }
\def\pst@rottable{%
@0=%
@U=%
@L=90 %
@D=180 %
@R=-90 %
@N=\pst@rotlist
@W=\pst@rotlist 90 add %
@S=\pst@rotlist 180 add %
@E=\pst@rotlist 90 sub }
%
\define@key[psset]{pstricks}{rot}[0]{%
  \pst@expandafter{\@ifnextchar*{\psset@@@rot}{\psset@@rot}}{#1}\@nil}
\def\psset@@rot#1\@nil{%
  \def\next##1@#1=##2@##3\@nil{%
    \ifx##2\relax\pst@getangle{#1}\psk@rot \else\def\psk@rot{##2}\fi%
    \pst@Verb{ gsave  STV CP T /ps@rot \ifx\psk@rot\@empty 0 \else \psk@rot \fi def grestore }% (MJS)
  }%
  \expandafter\next\pst@rottable @#1=\relax @\@nil}
%
\def\psset@@@rot#1#2\@nil{%
  \psset@@rot#2\@nil%
  \edef\psk@rot{\pst@rotlist \ifx\psk@rot\@empty\else\space ps@rot add \fi}%
  \pst@Verb{ gsave  STV CP T /ps@rot \ifx\psk@rot\@empty 0 \else \psk@rot \fi def grestore }}% (MJS)
%
%\def\psset@@rot#1\@nil{%
%\def\ps@next##1@#1=##2@##3\@nil{%
%\ifx\relax##2\pst@getangle{#1}\psk@rot\else\def\psk@rot{##2}\fi}%
%\expandafter\ps@next\pst@rottable @#1=\relax @\@nil}
%
%\def\psset@@@rot#1#2\@nil{%
%\psset@@rot#2\@nil
%\edef\psk@rot{\pst@rotlist \ifx\psk@rot\@empty\else\psk@rot add \fi}}
\psset[pstricks]{rot=0}
%
\def\tx@RotBegin{RotBegin }
\def\tx@RotEnd{RotEnd }
\def\pst@rotate#1#2{%
  \ifx#1\@empty\else
  \setbox#2=\hbox{\pst@Verb{#1 \tx@RotBegin}\box#2\pst@Verb{\tx@RotEnd}}%
  \fi%
}
\def\psput@cartesian#1{%
  \hbox to \z@{\kern\pst@dimg{\vbox to \z@{\vss\box#1\vskip\pst@dimh}\hss}}%
}
\def\psput@special#1{%
  \hbox{%
    \pst@Verb{{ \pst@coor \pstnodescale } \tx@PutCoor \tx@PutBegin }%
    \box#1%
    \pst@Verb{ \tx@PutEnd }%
  }%
}
\def\tx@PutCoor{PutCoor }
\def\tx@PutBegin{PutBegin }
\def\tx@PutEnd{PutEnd }
\def\rput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\rput@i}{\rput@ii}}}
\def\rput@i[#1]{\addto@par{ref={#1}}\rput@ii}
\def\rput@ii{\@ifnextchar({\rput@iv}{\rput@iii}}
\def\rput@iii#1{\addto@par{rot={#1}}\@ifnextchar({\rput@iv}{\rput@iv(\z@,\z@)}}
\def\rput@iv(#1){\pst@killglue\pst@makebox{\rput@v{#1}}}
\def\rput@v#1{%
  \begingroup%
    \use@par%
    \if@star\pst@starbox\fi%
    \pst@makesmall\pst@hbox%
    \ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% (MJS)
%    \pst@rotate\psk@rot\pst@hbox%
    \psput@{#1}\pst@hbox%
  \endgroup%
  \ignorespaces}
%
\def\multirput{%
  \def\pst@par{}%
  \pst@ifstar{\@ifnextchar[{\multirput@i}{\multirput@ii}}}
\def\multirput@i[#1]{\addto@par{ref={#1}}\multirput@ii}
\def\multirput@ii{\@ifnextchar({\multirput@iv}{\multirput@iii}}
\def\multirput@iii#1{\addto@par{rot={#1}}\multirput@iv}
\def\multirput@iv(#1){%
  \@ifnextchar({\multirput@v(#1)}{\multirput@v(\z@,\z@)(#1)}}
\def\multirput@v(#1,#2)(#3,#4)#5{%
  \pst@makebox{\multirput@vi(#1,#2)(#3,#4){#5}}}
\def\multirput@vi(#1,#2)(#3,#4)#5{%
  \pst@killglue%
  \global\psLoopIndex=\@ne\relax
  \begingroup
    \use@par
    \if@star\pst@starbox\fi
    \pst@makesmall\pst@hbox
    \ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% (MJS)
%    \pst@rotate\psk@rot\pst@hbox
    \pssetxlength\pst@dima{#1}%
    \pssetylength\pst@dimb{#2}%
    \pssetxlength\pst@dimc{#3}%
    \pssetylength\pst@dimd{#4}%
    \pst@cntg=#5\relax
    \leavevmode
    \loop
      \vbox to \z@{%
        \vss
        \hbox to \z@{\kern\pst@dima\copy\pst@hbox\hss}%
        \vskip\pst@dimb%
      }%
      \ifnum\pst@cntg>\psLoopIndex
        \advance\pst@dima\pst@dimc
        \advance\pst@dimb\pst@dimd
        \global\advance\psLoopIndex by \@ne
    \repeat 
  \endgroup
  \ignorespaces%
}
%
\newif\if@fixedradius
\def\cput{\def\pst@par{}\pst@object{cput}}
\def\cput@i{\@fixedradiusfalse\cput@ii}
\def\cput@ii{\pst@killglue\@ifnextchar({\cput@iv}{\cput@iii}}
\def\cput@iii#1{%
  \addto@par{rot={#1}}%
  \@ifnextchar({\cput@iv}{\cput@iv(\z@,\z@)}%
}
\def\cput@iv(#1){\pst@makebox{\cput@v{#1}}}
  \def\cput@v#1{%
  \begingroup
    \use@par
    \setbox\pst@hbox=\hbox{%
      \psboxsepfalse
      \if@fixedradius\psCirclebox@ii\else\pscirclebox@ii\fi%
    }%
    \pst@@makesmall\pst@hbox
    \ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% (MJS)
%    \pst@rotate\psk@rot\pst@hbox
    \psput@{#1}\pst@hbox
  \endgroup
  \ignorespaces%
}
%
\def\Cput{\def\pst@par{}\pst@object{Cput}}
\def\Cput@i{\@fixedradiustrue\cput@ii}
\newdimen\pslabelsep
\define@key[psset]{pstricks}{labelsep}[5pt]{%
  \pssetlength\pslabelsep{#1}%
  \ifx\PSTplotLoaded\endinput% Set labels for pst-plot, if laoded
    \let\psxlabelsep\pslabelsep%
    \let\psylabelsep\pslabelsep%
  \fi}
\psset[pstricks]{labelsep=5pt}
%
\define@key[psset]{pstricks}{refangle}[0]{\pst@expandafter\psset@@refangle{#1}\@nil}
\def\psset@@refangle#1\@nil{%
  \def\next##1@#1=##2"##3@##4\@nil{%
    \ifx\relax##2%
      \pst@getangle{#1}\psk@refangle
      \def\psk@uputref{}%
    \else
      \def\psk@refangle{##2 }%
      \def\psk@uputref{##3}%
    \fi}%
  \expandafter\next\pst@refangletable @#1=\relax"@\@nil%
  \pst@Verb{ gsave STV CP T /ps@refangle \psk@refangle\space def grestore }%ADDED (MJS)
}
%
\def\pst@refangletable{%
@r=0"20%
@u=90"02%
@l=180"10%
@d=-90"01%
@ur=45"22%
@ul=135"12%
@dr=-135"21%
@dl=-45"11}
\psset[pstricks]{refangle=0}

% DG/SR modification begin - Mar. 24, 1999 - Patch 10
%\def\uput{\def\pst@par{}\@ifnextchar[{\uput@ii}{\uput@i}}
\def\uput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\uput@ii}{\uput@i}}} 
% DG/SR modification end
\def\uput@i#1{\addto@par{labelsep=#1}\uput@ii}
\def\uput@ii[#1]{%
  \addto@par{refangle={#1}}%
  \@ifnextchar({\uput@iv}{\uput@iii}}
\def\uput@iii#1{%
  \addto@par{rot={#1}}%
  \@ifnextchar({\uput@iv}{\uput@iv(\z@,\z@)}}
\def\uput@iv(#1){\pst@killglue\pst@makebox{\uput@v{#1}}}
\def\uput@v#1{%
  \begingroup
  \use@par
  \if@star\pst@starbox\fi
  \pstCheckCoorType{#1}% needed for \uput@vii
  \uput@vi
  \psput@{#1}\pst@hbox
  \endgroup
  \ignorespaces}
%
\def\uput@vi{%
  \ifx\psk@uputref\@empty\uput@vii\tx@UUput{}%
  \else
    \ifx\psk@rot\@empty\expandafter\uput@viii\psk@uputref
    \else\uput@vii\tx@UUput{}\fi
  \fi}
% 
\def\uput@vii#1#2{%
  \edef\pst@coor{%
    \ifPst@SpecialLength \pst@SpecialLength \else \pst@number\pslabelsep \fi
%    \pst@number\pslabelsep % \ifdim\pslabelsep<\z@  neg \fi
    #2%
    \pst@number{\wd\pst@hbox}%
    \pst@number{\ht\pst@hbox}%
    \pst@number{\dp\pst@hbox}%
    \ifnum\pst@C@@rType=7\relax
      ps@refangle % CHANGED (MJS) FROM \psk@refangle\space
      \ifx\psk@rot\@empty\else ps@rot\space sub \fi
    \else
      \psk@refangle\space 
      \ifx\psk@rot\@empty\else \psk@rot\space sub \fi
    \fi
    \tx@Uput #1}%
    %\show\pst@coor
  \setbox\pst@hbox=\hbox to\z@{\hss\vbox to\z@{\vss\box\pst@hbox\vss}\hss}%
  \setbox\pst@hbox=\psput@special\pst@hbox
  \ifnum\pst@C@@rType=7\relax
    \ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% CHANGED FROM \psk@rot (MJS)
  \else
    \ifx\psk@rot\@empty\else\pst@rotate{\psk@rot}\pst@hbox\fi% 
  \fi}
%
%
\def\uput@viii#1#2{%
  \ifnum#1>\z@\relax\ifnum#2>\z@\relax\pslabelsep=.707\pslabelsep\fi\fi
  \setbox\pst@hbox=\vbox to\z@{%
    \ifnum#2=1\relax\vskip\pslabelsep\else\vss\fi
    \hbox to\z@{%
      \ifnum#1=2\relax\hskip\pslabelsep \else\hss\fi
      \box\pst@hbox%
      \ifnum#1=1\relax\hskip\pslabelsep\else\hss\fi}%
    \ifnum#2=2\relax\vskip\pslabelsep\else\vss\fi}}
%
\def\tx@Uput{Uput }
\def\tx@UUput{UUput }
%
\def\Rput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Rput@ii}{\Rput@i}}}
\def\Rput@i#1{\addto@par{labelsep=#1}\Rput@ii}
\def\Rput@ii[#1]{\addto@par{ref={#1}}\@ifnextchar({\Rput@iv}{\Rput@iii}}
\def\Rput@iii#1{\addto@par{rot={#1}}\@ifnextchar({\Rput@iv}{\Rput@iv(\z@,\z@)}}
\def\Rput@iv(#1){\pst@killglue\pst@makebox{\Rput@v{#1}}}
\def\Rput@v#1{%
  \begingroup
  \use@par
  \if@star\pst@starbox\fi
  \Rput@vi
  \pst@makesmall\pst@hbox
  \ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% (MJS)
%  \pst@rotate\psk@rot\pst@hbox
  \psput@{#1}\pst@hbox
  \endgroup
  \ignorespaces}
%
\def\Rput@vi{%
  \pst@dimg=\dp\pst@hbox
  \advance\pst@dimg\pslabelsep
  \dp\pst@hbox=\pst@dimg
  \pst@dimg=\ht\pst@hbox
  \advance\pst@dimg\pslabelsep
  \ht\pst@hbox=\pst@dimg
  \setbox\pst@hbox\hbox{\kern\pslabelsep\box\pst@hbox\kern\pslabelsep}}%
%
\def\oldpsput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\oldpsput@i}{\oldpsput@ii}}}
\def\oldpsput@i[#1]{\addto@par{ref={#1}}\oldpsput@ii}
\def\oldpsput@ii{\@ifnextchar<{\oldpsput@iii}{\oldpsput@iv}}
\def\oldpsput@iii<#1>{\rput@iii{#1}}
\def\OldPsput{\let\psput\oldpsput}
\def\NewPsput{\let\psput\rput}
%
% -----------  hv 20120219 -------------------
\newpsstyle{gridstyle}{subgriddiv=0,gridcolor=lightgray,griddots=10,gridlabels=8pt}
\newpsstyle{gridstyleA}{subgriddiv=5,gridcolor=red!30,subgridcolor=green!20!black!10,gridlabels=0pt}
%\define@boolkey[psset]{pstricks}[]{showgrid}[true]{}
\newif\ifshowgrid
\newdimen\sh@wgridXunit
\newdimen\sh@wgridYunit
\define@key[psset]{pstricks}{showgrid}[b]{\expandafter\pst@@showgrid#1!!\@nil}
\def\pst@@showgrid#1#2#3\@nil{%                            hv 20130403
  \def\showgridp@s{0}%
  \ifx#1b\showgridtrue\else%                               bottom
    \ifx#1f\showgridfalse\else%
      \ifx#1t%
        \ifx#2r\showgridtrue\else%  			   true->bottom
               \showgridtrue\def\showgridp@s{1}\fi%        top
  \fi\fi\fi%
  \ifnum\showgridp@s>0
    \sh@wgridXunit=\psxunit%
    \sh@wgridYunit=\psyunit%
  \fi%
}
\psset[pstricks]{showgrid=false}
\define@boolkey[psset]{pstricks}[Pst@]{pgffunctions}[true]{}
\psset[pstricks]{pgffunctions=false}
%
\newdimen\pst@shift
\newif\ifPst@shift@star
\define@key[psset]{pstricks}{shift}[0]{%
  \ifx#1*
    \global\Pst@shift@startrue
    \pst@shift=\p@
  \else
    \global\Pst@shift@starfalse
    \pssetlength\pst@dimg{#1}
    \global\pst@shift\pst@dimg%   only the outer pspicture env can have a shift
  \fi}
\psset[pstricks]{shift=0}
%
%------------------------------- pspicture ------------------------------
%
\def\pspicture{\begingroup\pst@ifstar\pst@picture}
\def\pst@picture{\@ifnextchar[{\pst@@picture}{\pst@@picture[]}}
\def\pst@@picture[#1]{\@ifnextchar({\pst@@picture@i[#1]}{\pst@@picture@i[#1](10,10)}}%
\def\pst@@picture@i[#1]#2(#3,#4){\@ifnextchar(%   ignore anything between [] and ()
  {\pst@@@picture[#1](#3,#4)}%
  {\pst@@@picture[#1](0,0)(#3,#4)}}
%
\def\pst@@@picture[#1](#2,#3)(#4,#5){%
  \pssetxlength\pst@dima{#2}%
  \pssetylength\pst@dimb{#3}%
  \pssetxlength\pst@dimc{#4}%
  \pssetylength\pst@dimd{#5}%
  \ifdim\pst@dima>\pst@dimc%
    \pst@dimg=\pst@dima%
    \pst@dima=\pst@dimc%
    \pst@dimc=\pst@dimg%
  \fi%
  \ifdim\pst@dimb>\pst@dimd%
    \pst@dimg=\pst@dimb%
    \pst@dimb=\pst@dimd%
    \pst@dimd=\pst@dimg%
  \fi%
  \setbox\pst@hbox=\hbox\bgroup%
  \begingroup\KillGlue%
  \@ifundefined{@latexerr}{}{\let\unitlength\psunit}%
  \edef\pic@coor{(#2,#3)(#2,#3)(#4,#5)}%
% ----------- 1.10/12 beg hv -------------------
  \psset{showgrid=false}%                % for nested pspicture environemnets
  \def\pst@tempA{#1}%
  \ifx\pst@tempA\@empty\else\psset{#1}\fi% sets the shift and grid option
  \ifx\pst@bgcolor\@empty \else\psframe*[linecolor=\pst@bgcolor](#2,#3)(#4,#5)\fi
  \ifshowgrid\ifnum\showgridp@s=0\psgrid[style=gridstyle]\fi\fi%
% ----------- 1.10/12 end hv -------------------
  \ignorespaces%			% 2008-12-07
  \ifPst@pgffunctions\pstVerb{ pgffunctions } \fi % hv 2013-04-17
}
\def\pic@coor{(0,0)(0,0)(10,10)}
%\newdimen\pst@shift
\def\endpspicture{%
  \ifshowgrid\ifnum\showgridp@s>0
    \psgrid[xunit=\sh@wgridXunit,yunit=\sh@wgridYunit,style=gridstyle]\fi\fi%
  \pst@killglue
%  \global\pst@shift=\pst@shift% in fact of the following endgroup
  \endgroup
  \egroup
  \ifdim\wd\pst@hbox=\z@\else
    %\@pstrickserr{Extraneous space in the pspicture environment}%
    %{Type \space <return> \space to proceed.}%
  \fi
  \ht\pst@hbox=\pst@dimd
  \dp\pst@hbox=-\pst@dimb
  \setbox\pst@hbox=\hbox{%
    \kern-\pst@dima
% Orig version ----------
%\ifx\pst@tempa\@empty\else
%\advance\pst@dimd-\pst@dimb
%\pst@dimd=\pst@tempa\pst@dimd
%\advance\pst@dimd\pst@dimb
%\lower\pst@dimd
%\fi
%----- end Orig
    \ifPst@shift@star%\typeout{==pstricks== old behaviour of the shift option}%     shift=*
      \advance\pst@dimd-\pst@dimb
      \pst@dimd=0.5\pst@dimd
    \else\pst@dimd-\pst@shift\fi
    \advance\pst@dimd\pst@dimb
    \lower\pst@dimd%
    \box\pst@hbox%
    \kern\pst@dimc}%
  \if@star\setbox\pst@hbox=\hbox{\clipbox@@\z@}\fi%
  \leavevmode\box\pst@hbox%
  \endgroup%
  \psset[pstricks]{shift=0}% reset value
}
%
\@namedef{pspicture*}{\pspicture*}
\@namedef{endpspicture*}{\endpspicture}
%
\ifx\pstcustomize\relax \input pstricks.con \fi
\catcode`\@=\PstAtCode\relax
%
\endinput
%%
%% END: pstricks.tex

